Farview: Disaggregated Memory with Operator Off-loading for Database Engines

Cloud deployments disaggregate storage from compute, providing more flexibility to both the storage and compute layers. In this paper, we explore disaggregation by taking it one step further and applying it to memory (DRAM). Disaggregated memory uses network attached DRAM as a way to decouple memory from CPU. In the context of databases, such a design offers significant advantages in terms of making a larger memory capacity available as a central pool to a collection of smaller processing nodes. To explore these possibilities, we have implemented Farview, a disaggregated memory solution for databases, operating as a remote buffer cache with operator offloading capabilities. Farview is implemented as an FPGA-based smart NIC making DRAM available as a disaggregated, network attached memory module capable of performing data processing at line rate over data streams to/from disaggregated memory. Farview supports query offloading using operators such as selection, projection, aggregation, regular expression matching and encryption. In this paper we focus on analytical queries and demonstrate the viability of the idea through an extensive experimental evaluation of Farview under different workloads. Farview is competitive with a local buffer cache solution for all the workloads and outperforms it in a number of cases, proving that a smart disaggregated memory can be a viable alternative for databases deployed in cloud environments.

==> chapters/chapters_asplos/background.tex <==
\section{Background and Related Work}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/intro2.pdf}
\caption{Disaggregated DRAM, added layer in a data center}
\label{fig:intro}
\end{figure}

 %To define the scope of the paper and put our results in perspective, it is important to distinguish among the many different versions of disaggregated, remote, persistent memory, etc. that modern hardware is enabling and also to justify the design choices made in Farview. 

\subsection{The Need for More Memory}

%The main motivation for this paper is the increasing demand for memory capacity in data centers and the cloud.

The rising popularity of in-memory workloads such as machine learning, key-value stores, and in-memory analytics has caused memory demands in compute clusters to grow rapidly~\cite{Barroso18}. This growing demand for in-memory computing, coupled with the slowdown of device scaling~\cite{Lee16}, has led to the DRAM becoming a major bottleneck in data centers~\cite{FacebookNVM18, GoogleFarMemory19}.
To address this need, approaches leverage advances in memory technologies and networking to increase effective DRAM capacity.
Within the local node, studies have explored compressing cold pages into local DRAM~\cite{GoogleFarMemory19} or
using local NVM directly as memory or with DRAM acting as a transparent caching layer~\cite{Octane19,Octane19-b,HybridMem16}.

Networking advances were explored to expand the available virtual memory using memory outside the local machine.
In the following sections we will provide an overview of these networking advances, as well as summarize approaches for non-local memory.
Many of these ideas are not strictly new:
the notions that memory and storage can be active, rather than passive, components
and can be shared across a cluster of machines
have been around for decades \cite{TreadMarks96,ActivePages98,IDisks98,IRAM97,PatRAM97}.
However, technology has changed in major ways and the advent of in-memory, big-data use cases has made the need for expanding main memory more urgent. 

\subsection{Network Technology Advances}

Data center network speed and efficiency have improved dramatically in the last decade.
Today, it is common for data center networks to provide 40 Gbps per server~\cite{Facebook13, AzureAccel16}, with increases to 100Gbps per server visible on the horizon~\cite{Facebook19}.
Network latency has also improved considerably, with one-way switch latencies in the sub-microsecond range~\cite{Mellanox19}.

To minimize the processing overheads of traditional TCP/IP protocols, many networks have adopted Remote Direct Memory Access (RDMA)~\cite{Alibaba20,catapult2.0}. % note: AzureAccel16 == catapult2.0, 
RDMA is
%, or its implementations in the form of a RoCE (RDMA-over-converged-Ethernet) or Infiniband stack, are 
used through verbs that enable one-sided and two-sided operations (without or with intervention of the remote CPU, respectively) as well as atomic operations on remote memory locations and zero-copy large data transfers directly to/from a machine's memory. 
% zero-copy, completely offloaded transfers of large amounts of data directly to/from the memory of a machine
%RDMA provides both one-sided operations, which allow one machine to directly read and write memory in a remote machine without remote CPU intervention, and two-sided operations, which permit traditional messages that engage both the sender and receiver CPU.
RDMA-based reads and writes to a remote node can be performed within single-digit microseconds~\cite{Farm14,FarMemory20,Strom20,AsymNVM20}.

While RDMA improves the bandwidth limitations of non-local memory, the issue of latency when compared with NVM or DRAM remains. Typically, latency is hidden through techniques such as caching and batching. Additionally, smart NICs are increasingly recognized as a way to tailor the network communication to the needs of the application or to reduce the impact of networking on overall performance. For instance, Microsoft has offloaded network management to a smart NIC~\cite{catapult3.0}, and offers the opportunity to offload other functionality to the NIC~\cite{catapult1.0,catapult2.0}. Smart NICs are also used as hardware acceleration of application logic, typically acting on data as it flows through the network, which minimizes the application changes required~\cite{Strom20,Lynx20,KVdirect}.
%From the application side, a smart NIC allows hardware acceleration of many different applications without necessarily requiring major changes to those applications, as it typically acts on the data as it flows through the network card~\cite{Strom20,Lynx20,KVdirect}.
% KK: what functionality do the catapult1/2 refs allow users to offload?

\subsection{Non-local Memory Alternatives}

Multiple system organizations, including remote memory and disaggregated memory, leverage RDMA and smart NIC technologies to augment local memory.

% KK note: The AsymNVM folks call remote memory "symmetric" and disaggregated "asymmetric".

% \textit{Remote memory} is a shared, distributed memory infrastructure that makes the DRAM memory resident at a pool of machines available to other machines. Remote memory resides on machines that are comparably equipped (e.g., with a processor, local memory, local storage) to the compute node where the application needing more memory runs. 
\textit{Remote memory} is a shared, distributed memory infrastructure where a group of comparably equipped (e.g., with a processor, local memory, local storage) compute nodes make their memory available to their peers.
This organization has the advantage of not requiring any additional resources and, theoretically, improves resource utilization by taking advantage of unused memory across a group of machines. 
%\cite{TreadMarks96,RemoteMemory17,FarMemory20}, i.e., 
Previous systems have presented remote memory to applications as a remote paging device~\cite{FarMemory20, Infiniswap17}, as a file system~\cite{RemoteMemory18}, and as distributed shared memory~\cite{Farm14, Grappa15, Hotpot17}.

However, remote memory has several potential drawbacks: a) it does not allow scaling compute and memory capacity independently, thereby increasing cost; b) it does not increase the memory capacity if all servers are active at the same time~\cite{Blades09}; c) it assumes the memory in other machines is unused, which is not always true, and makes managing the overall availability including tail latency, a difficult problem~\cite{GoogleFarMemory19}; d) it expands the failure domain and attack surface of each machine, leading to application failures and vulnerabilities~\cite{GoogleFarMemory19, RemoteMemory17}.


%However, in a data center or cloud setting, remote memory has several potential drawbacks. First, adding more remote memory means also adding more compute nodes, which increases costs and does not allow scaling compute and memory capacity independently. Second, remote memory does not really increase the memory capacity since the compute:memory ratio remains the same if all servers are active at the same time~\cite{Blades09}. Third, remote memory assumes the memory in other machines is unused, which is not always true, and makes managing the overall availability of remote memory, including tail latency, a difficult problem~\cite{GoogleFarMemory19}. Finally, remote memory expands the failure domain of each machine, increasing the likelihood that a portion of an application's memory resident data becomes unavailable and leading to application failures~\cite{GoogleFarMemory19}. It also increases the attack surface of each computing node to include vulnerabilities of the remote machines~\cite{RemoteMemory17}.
% KK: not sure I buy this last argument.
%Finally, although rarely stated explicitly, remote memory makes sense mostly for centralized applications. Distributed systems commonly used to process big data (e.g., Spark) do not benefit from remote memory since they are already distributed and, thus, already leverage the memory resources available at different machines. In those cases, which are mostly the use cases we target, it is not clear what remote memory would add since, if the data is in the memory of another computing node, it is typically better to ship a worker to process the data in-situ than to move the data. 

Alternatively, \textit{disaggregated memory} systems use network attached memory that is distinct from the memory in the compute nodes~\cite{Dis12}. Figure~\ref{fig:intro} illustrates this organization. 
%Thus, a separate pool of memory is made available to computing nodes so that they can dynamically expand the capacity of their local memory 
Disaggregated memory can be scaled independently of the computing or storage capacity of the system~\cite{Blades09}. As a result, it offers the possibility of increasing the efficiency of clusters and data centers by removing the need for memory over-provisioning at each computing node (or by adding unnecessary computing nodes only for their memory). It is easier to allocate, share and manage than memory residing in machines that are also performing other computations. Furthermore, data can be easily encrypted (as we will show) to address the security concerns around remote memory~\cite{GoogleFarMemory19} when the data is stored in machines where other users are running active computations.
%(something that would require remote CPU resources for remote memory).

Previous disaggregated architectures have presented their memory as byte-addressable regions that preserve the load/store interface of conventional memory (e.g., The Machine from HPE~\cite{TheMachine1,TheMachine2}, which uses Gen-Z~\cite{GenZ,Knebel19} rather than RDMA), as a paging device~\cite{Blades09,Dis12}, as a persistent key-value store (e.g., FlatStore~\cite{FlatStore20}, Clover~\cite{pDPM20}), as a database storage engine~\cite{Binnig16}, as a persistent memory file system (e.g., Octopus~\cite{Octopus17}, Orion~\cite{Orion19}), or as recoverable persistent data structures (e.g., AsymNVM~\cite{AsymNVM20}).
% KK note: Kevin Lim's work (Blades09, Dis12) doesn't use RDMA -- it uses PCIe and HyperTransport coherent interconnect

% KK note: may want to say more about how much intelligence is assumed on the disaggregated memory nodes. Yiying Zhang's group at UCSD distinguishes between "passive" (dumb: no data processing or metadata operations) and "active" (smart: some data processing and/or metadata operations)

% KK note: may want to say more about specifics of how these systems try to compensate for latency of remote/disaggregated memory access
%For instance, \cite{AsymNVM20} uses back-end nodes with large amounts of NVM to implement byte-addressable remote memory with the argument that the bandwidth of NVM is similar to that of Infiniband networks and, thus, it is possible to use NVM remotely without bandwidth loss. To compensate for the latency differences (100s of ns for NVM vs single digit $\mu$s  for RDMA) the authors propose batching and caching on the computing nodes as well as assuming that the application's working set is cached in the local memory.

% KK note: we could elaborate here on limitations to RDMA, based on discussion in LITE-SOSP17, RemoteRegions-ATC18.
% KK note: we could also use the RDMA limitations to motivate the reason that people use higher level APIs for their disaggregated systems.
Despite RDMA's performance wins, its low-level verbs interface can be too restrictive for many memory-centric applications, leading to proposed extensions that raise the level of abstraction.
% provided by both remote and disaggregated memory
Far memory~\cite{FarMemory20} proposes hardware extensions (e.g., indirect addressing modes, scatter/gather support) to reduce the number of network traversals to access non-local memory, as well as support for efficient notifications to facilitate consistency of data in local memory.
% KK: should we also include LITE from SOSP17?
HyperLoop~\cite{Hyperloop18}, AsymNVM~\cite{AsymNVM20}, and StRoM~\cite{Strom20} extend one-sided operations on RDMA smart NICs to include additional system-level and application-level logic.
HyperLoop offloads group-based operations to RDMA NICs to support traditional storage functions like replicating data and managing replicated logs.
AsymNVM offloads point-to-point persistent memory allocation, concurrency and transaction functionality.
StRoM offloads point-to-point memory access operations like indirect addressing for remote data structure traversal, data shuffling, and cardinality estimation to support distributed key-value store applications.

\subsection{Target Environment}
In this paper, we target RDMA-based disaggregated DRAM systems, exploring memory abstractions that compensate for network latency issues using 
%Dejan changed original "memory-side near-data processing operators"
memory-side data operators
that reduce network traversals and the amount of data sent across the network and save work at the requesting computing node. For this purpose, the disaggregated memory needs to become smart and support advanced features such as complex addressing modes, data filtering, and data transformations that allow it to offer more than conventional memory. Because a smart NIC is a simple and efficient way to implement such a smart disaggregated memory, we follow on from previous work~\cite{Hyperloop18, AsymNVM20, Strom20} and extend RDMA one-sided verbs to enable a more sophisticated interaction with the disaggregated memory. 
In comparison to these works, memory views provide a richer set of application-level operators (addressing, filtering and transformation) for disaggregated memory.
Additionally, the Farview platform provides concurrent access through different views, and supports dynamic runtime reconfiguration of the FPGA regions that implement operators.

%\todo{\textit{TODO: Be more explicit about why we're choosing DRAM rather than NVM. Suggest pushing comparison between Farview and StRoM to the Farview section.}}

==> chapters/chapters_asplos/conclusion.tex <==
\section{Conclusions}

%We have explored the possibility of implementing smart disaggregated DRAM by using RDMA and a smart NIC. Through a number of examples and a comprehensive performance evaluation, %facilitated by Farview, an open source platform designed to study memory models, 
%we demonstrate the potential of the idea and the several ways in which it can be used to improve application performance  or data center efficiency by reducing the pressure on the DRAM of computing nodes. Future work will include expanding the range of operators, combining Farview with smart NICs on the client side, and developing complete applications that exploit smart disaggregated memory. 
%In the long-term we will explore support for NVM and scaling Farview to emulate larger memory systems.
%and scaling Farview to multiple (cooperating) instances per node and across multiple nodes.
% KK: "per node" is confusing, as we've talked about our vision of disaggregated memory as not being associated with a (compute) "node". If we're talking about the Farview platform, I think this may leave doubts in reviewers' minds about how scalable our system is.

We have explored a view abstraction for smart disaggregated memory, which applies addressing, filtering and transformation operations to disaggregated memory-resident data.
We present Farview, an  open  source  platform for  studying  novel network-attached memory system that extends RDMA one-sided verbs to implement view operators.
Our experiments show that this approach improves the performance of data-centric processing, outperforming more traditional one-sided and two-sided RDMA alternatives. 
Future work will include expanding the range of operators, combining Farview with smart NICs on the client side, and developing complete applications that exploit smart disaggregated memory. 


==> chapters/chapters_asplos/evaluation.tex <==
\section{Implementation setup}
\label{sec:eval}

%To explore the potential of disaggregated DRAM memory, we have used Farview to implement a number of operators providing a variety of views to the client nodes. These views test the ideas described and give more information on how such a system would operate. 

We have implemented Farview on a Xilinx VCU118 board with an Ultrascale+ VU9P FPGA chip. The FPGA is attached to the host CPU via a PCIe x16 slot. The board has 2 DRAM banks (8GB each), connected directly to the FPGA. Each DDR channel has a softcore (running as reconfigurable logic on the FPGA) DRAM controller with a theoretical bandwidth of 18GB/s. The board has two (QSFP) 100Gbps network ports. % The boards are directly connected to each other through one of the two available QSFP (or network) ports. 
The host CPU is an 8 core Intel i5-4590 CPU base clocked at 3.3 GHz. Code compilation for the CPU baselines was done with -O3 optimization flag and AVX2 instructions were used where applicable. We compare Farview to both one-sided and two-sided RDMA operations.
Our baseline system (called "cNIC" in the results) uses a commercial Mellanox 100G card (ConnectX-5 VPI) \cite{melanoxCard}.

% For a real world case we use the system with a commercial 100G NIC.

\subsection{Resource utilization}

We use six dynamic regions in our experiments; Farview has been tested with up to ten regions, the empirical limit for our device. Farview does not require a large amount of resources, even considering that it contains the entire management logic, all the dynamic regions, the network stack, and the memory controller. The resources used for the deployed system on the FPGA are shown in Table \ref{table:resource_shell}. Farview does not utilize more than 25 \% of the total on-chip resources.  The majority of the utilized on-chip memory is caused by the memory management unit and the state keeping structures of the network stack. Additionally, most of the implemented operators are not compute heavy and do not take many resources which makes it easy to combine them and enables the support for more dynamic regions.

%The exceptions are operators like decision tree inference and count min which utilize sizeable amount of special compute blocks (DSPs and BRAM). 

\begin{table}[t!]
\centering
\caption{Resource overhead of the Farview}
\label{table:resource_shell}
\begin{scriptsize}
\centering
%\begin{tabular}{c|c|c|c|c}
\begin{tabular}{l|r|r|r|r}
\textbf{Configuration} & \textbf{CLB LUTs} & \textbf{Regs} & \textbf{BRAM tiles} & \textbf{DSPs} \\
\hline
\textit{6 regions} & 24\% & 23\% & 19\% & 0\% \\
\hline
\textbf{Operators} & \textbf{CLB LUTs} & \textbf{Regs} & \textbf{BRAM tiles} & \textbf{DSPs} \\
\hline
\textit{Hash, Striding (each)} & $<$1\% & $<$1\% & 0\% & 0\% \\
\textit{Matrix transposition} & $<$1\% & $<$1\% & 12\% & 0\% \\
\textit{Reduced prec., Selection (each)} & $<$1\% & $<$1\% & 2\% & 0\% \\
\textit{Average, Sum (each)} & $<$1\% & $<$1\% & 0\% & 0\% \\
\textit{AES encryption} & 3.6\% & $<$1\% & 0\% & 0\% \\
\textit{Regex} & 1.1\% & $<$1\% & 0\% & 0\% \\
\end{tabular}
\end{scriptsize}
\end{table}

\section{Farview Microbenchmarks}

%Modern FPGAs are usually equipped with a growing amount of local, FPGA attached memory \cite{u250} and some experimental systems have announced up to 512 GB of local memory on the FPGA \cite{Enzian20}. This memory provides better performance than memory attached over PCIe. Multiple banks are usually present offering additional parallelization potential, a crucial advantage in the type of workloads targeted by Farview.
In this section we evaluate the performance of the Farview evaluation platform. We begin by creating an approximation roofline model explaining the platform's limitations. We then measure the overhead for loading dynamic operators and evaluate the RDMA performance of the Farview and baseline systems. Finally, we examine Farview's concurrency and the bandwidth distribution between regions.

\subsection{Roofline Model}

\input{graphs/roofline}

To put Farview in perspective, %Dejan shortened: and also as a useful reference for other technologies and approaches,% 
we have developed a roofline model based on: DRAM, network, PCIe, and ability to compute on the FPGA (Figure \ref{fig:roofline}). The X-axis represents the operational intensity required to perform a task (the number of operations/cycle over the number of bytes/cycle) and the Y-axis represents operations/cycle. The model is assembled from different bandwidth ceilings measured on Farview and the maximum processing performance of the system. % Dejan shortened: Together, these define areas from which application behaviour can be inferred.

The computational bounds are calculated as follows. Each integer operation occupies ~20 lookup tables (LUTs) \cite{xilinxRoof}. The board used contains 1,182,240 lookup tables and is clocked at 250 MHz. The theoretical peak integer throughput is then 14.78 TOPS/s (Tera Operations per second). The size of a single dynamic region is 1/12 of the FPGA. This implies a maximum throughput of 1.23 TOPS/s per dynamic region. The upper performance bound depends on the number of regions used (horizontal blue lines in Figure \ref{fig:roofline} for 1 and 6 regions).

The bandwidth ceilings are established from the network, PCI interconnect, and the local memory (diagonal lines in Figure \ref{fig:roofline}). The 100 Gbps network has a ceiling around 12 GBps. The local FPGA memory can support up to 15 GBps ("DDR 1chan - 15 GBps" in Figure \ref{fig:roofline}), per channel, based on our measurements. The device in question has two separate memory channels that can be used together through the MMU, giving a total of 30 GBps ("DDR 2chan - 30GBps" in Figure \ref{fig:roofline}). We measured the PCIe bandwidth at 11 GBps. 

%Dejan shortened: From the roofline model we can derive important insights. 
The lines marking the regions indicate the maximum performance reachable with 1 or 6 dynamic regions. PCIe provides the lowest bandwidth, pointing to the limitations of remote memory approaches \cite{FarMemory20}. This is an important aspect in existing systems. For instance, AsymNVM \cite{AsymNVM20}, which uses NVM, uses Infiniband at 40 Gbps (5 GBps), thereby introducing a significant network bottleneck. Due to the use of PCIe, such a design will be bound by the PCIe even if network bandwidth increases. In Farview, which does not use PCIe, the main bandwidth bottleneck is the network. As the lines for memory show, if we use multiple memory channels, Farview is able to scale up to networks operating at 200 Gbps. Unlike other systems such as {StRoM} \cite{sidler2019innetworkdataprocessing}, the multiple dynamic regions in Farview allow to get closer to the network bandwidth by using more operators with high operational intensity concurrently. %  to support concurrent access to the disaggregated memory.  

%It is clear that the system in question is heavily under-provisioned in regards to memory bandwidth in comparison to the available computational resources. 

\input{graphs/system_sbs}

\subsection{Loading of the Operators}
\label{subsection:reconfig}

%\input{graphs/pr}

In Farview, operators provide different views over the data in the memory. These operators  can be loaded by clients at any point when accessing the disaggregated memory. The overhead of loading an operator is linear on the size of the deployed region implementing the operator. Table \ref{table:operator_load} shows the time required for regions of different sizes.

\begin{table}[t]
\centering
\caption{Time to dynamically load an operator}
\label{table:operator_load}
\begin{scriptsize}
\centering
%\begin{tabular}{c|c} 
\begin{tabular}{r|r} 
\textbf{Size of region [\% of FPGA]} & \textbf{Time [ms]} \\
\hline
6\% & 6.04 \\
12\% & 11.93 \\
33\% & 36.94 \\
66\% & 73.27 \\
\end{tabular}
\end{scriptsize}
\end{table}

\subsection{RDMA Throughput and Latency}



To characterize the system, we measure the network throughput and latency of RDMA read and RDMA write operations to the local FPGA memory. For reference and establishment of baselines we also provide the numbers for the setup where host memory over PCIe is accessed, giving an indication of how a smart NIC could operate in conjunction with remote memory (e.g., \cite{Strom20}). This setup is also used for all two-sided RDMA baselines where the processing is done in the back-end, on the remote CPU. The same measurements are reported for the commercial solution (cNIC) as well.

%The concurrency is then examined, first with the observation of the bandwidth distribution between dynamic regions when concurrent accesses are made and then with real-world examples where the benefit of having multiple regions is shown. We also present the roofline model with the application points, providing an intuitive visual aid in describing the system, its advantages and limitations.

Figures \ref{fig:thr_overlay_wr} and \ref{fig:thr_overlay_rd} show the median throughput for RDMA write and read operations. In the Farview case, a single dynamic region is present, accessing both the local and host (PCIe) memories, respectively. To obtain valid write measurements, the network round trip time (RTT) was measured and divided by two (RTT/2) over a series of 1000 runs. The transfer size represents the total data sent over the network for a single request. We vary this parameter until saturation is achieved. In the tests, packet size is set to 1 kB. The results show the typical under-saturation when using RDMA and the amount of data sent is not large enough. Up until the saturation point, the cNIC achieves better throughput, owing this to its specialized circuitry running at a higher clock rate which provides better performance for small packets. The results confirm the roofline model, reading or writing to the local FPGA memory peaks at 12 GBps, indicating that the network is the bottleneck. In both cases (cNIC and Farview-PCIe), where memory is accessed over PCIe, throughput peaks at \textasciitilde 11 GBps and is bound by the PCIe bus bandwidth.

%as benchmarked in a separate test. On the other hand, when FPGA memory is accessed, the throughput peaks at \textasciitilde 12 GBps. Although just slightly higher, it points to a different bottle-neck as separate memory benchmarks concluded the maximum throughput of \textasciitilde 15 GBps per channel for FPGA DRAM. The throughput scales linearly with the added channels. The bottle-neck in this case is thus the network stack and the 100G connection itself. The achieved throughput of \textasciitilde 96 Gbps is almost hitting the theoretical maximum. For concurrent processing the sheer advantage of local attached memory bandwidth provides significant advantage.

%In the following example, we place two applications directly on the READ and WRITE datapaths of the network streams and compare the performance to the case when basic READS and WRITES are issued. The biggest advantage here is the ability to fully pipeline the computation which adds negligible latency and does not affect performance. The overlay of the throughput with the processing and without it is present in Figure \ref{fig:rdma_op}.

%\input{graphs/rdma_op}

Figures \ref{fig:lat_measurements_wr} and \ref{fig:lat_measurements_rd} show the median latency for RDMA write and RDMA read operations. The benchmark setup is the same as for the throughput measurements. The results show the higher latency of accessing host memory over PCIe in comparison to accessing local FPGA memory. The difference during reads is \textasciitilde 1 us, consistent with reported PCIe latencies \cite{pcieLat}. The reduction is substantial (at least 20\%), again giving an indication of the advantages of implementing disaggregated memory with DRAM instead of with remote memory or NVM which at the moment require to use PCIe. The commercial NIC offers lower latencies for smaller transfer sizes, but this advantage disappears for higher transfer sizes where the more efficient multi-packet processing and page handling in the FPGA network stack shows its advantages.
The network round trip latency remains the dominating factor. The increase in latency is seen only above transfer sizes of 8 kB, caused by the amount of data.

\subsection{Multiple regions}

\input{graphs/fair_sharing}

\input{graphs/stride_sbs3}

Disaggregated memory has to provide balanced and fair access to concurrent clients. For this purpose, Farview incorporates a number of round-robing hardware arbitrators and a dedicated credit based system that result in an architecture very different form that of existing systems. To test it in practice, we execute concurrent RDMA read operations with 1 and 6 dynamic regions and measure the throughput. Figure \ref{fig:fair_sharing} shows the average throughput per region for different transfer sizes. As the graph shows, the bandwidth distribution is fair. When 6 memory bound operators access the memory concurrently, each one gets a sixth of the available bandwidth. The mean average deviation between the operators in these cases is negligible and demonstrates the fair-sharing between them. The same applies to the network access.



\section{Smart Addressing}

%In this section we present some of the implemented stateless non-blocking operators. These operators present a 1:1 mapping between the input and output \textcolor{blue}{Is hashing 1:1?} streams without any occurring state in between. As examples, we present two encryption and one hashing operators.

We now discuss views involving address translation without data modification. Unlike existing proposals for remote memory that follow a single pointer \cite{Farmemory19}, we expand the range and implement addressing modes used for NVM (Hash tables \cite{AsymNVM20}) and explore more complex views such as matrix transposition. These views support traversals of data structures at a reduced amount of network round trips and network requests.


%\input{graphs/rdma_indirect}

\subsection{Hash Table}

As a first example of indirect addressing and pointer traversal on disaggregated memory, we implement a typical hash table as used in, e.g., key-value stores, database indexes, and machine learning embeddings. The table uses Cuckoo hashing to resolve hash collisions. We use two hash functions, each one mapping entries to a different table. Each entry contains a pointer to the memory location where the values reside.

We compare the latency of a single one-sided GET operation executed on Farview vs. the commercial NIC for different value sizes and 64-bit keys (Figure \ref{fig:hash_table}). The median latency of 1000 completed requests is reported.

In the cNIC, at least two round trips are needed to fetch the values if the search operation is successful in the first attempt. If not, additional round trips are necessary \cite{Farm14,Strom20}. On Farview, we have developed an \textbf{HT} operator providing a view of the remote hash table that, upon receiving a key, performs the lookup, retrieves the value and sends it back in a single round trip regardless of the number of collisions.  For the test, accesses are uniformly distributed between the two hash tables which are placed in the same memory bank. The results demonstrate the effectiveness of smart disaggregated memory in reducing network latency for complex memory accesses as the latency is quite similar to that of a read operation given that the  \textbf{HT} operator is network bound. In contrast, conventional RDMA systems suffer from a growing overhead with collisions and data sizes. 

%\input{graphs/hash_table}


\subsection{Striding}

Many applications access data neither entirely sequentially nor completely at random. For instance, databases traverse large tables looking at particular attributes located in memory at regular intervals form each other. Such applications would benefit from a strided access interface. Scientific applications use strided access when performing column-major accesses to data stored in row-major order.
%The same when traversing large data collections where we are interested only in a few items placed at regular intervals. 
To support these applications, we have implemented a byte addressable \textbf{SA} operator able to read arbitrary spaced memory locations as if they were continuous, thus providing a large number of different data views to the clients. The interface exposes the following parameters: 1) \textit{Size}, the size of a single element, 2) \textit{Count}, the number of elements to fetch, 3) \textit{Stride}, the offset between elements. Any combination of these values is supported.

%\input{graphs/stride_sbs}
%\input{graphs/stride_sbs2}

Figure \ref{fig:striding_cmp} compares the latency when fetching elements in this way from disaggregated memory. In the figure, the offset between elements is set to 64 bytes, whilst the size of each element is 32-bits. We vary the number of total elements and measure the time to read all the items. The overhead of the basic RDMA read operation in the Farview is significant due to the redundant memory accesses. The Farview stride operator however, achieves a comparable (slightly better) performance compared to the commercial NIC using a single request for a whole data set through the network. The commercial NIC takes advantage of its ability to deal with small messages but at the price of having to flood the network with requests to fetch the complete data set and achieve comparable performance. 

The similar test setup is conducted in Figure \ref{fig:striding_mult} where 6 different users access remote memory concurrently using the Farview \textbf{SA} operator. This figure shows the comparison between the single and multiple dynamic regions present in the Farview. It shows a slight decrease and better efficiency in overall latency when multiple users and their requests are split among parallel dynamic regions, instead of the case when the same number of overall requests are submitted to one region.

%Additionally we examined the performance for different stride lengths; only a slight increase for large strides was observable, arising from the increased DRAM latency (random access) and is thus not shown. This operator is interesting because the gain is less obvious than in the previous cases. For small element sizes, the \textbf{SG} operator is clearly better, as it is memory bound while the RDMA READ is network bound. For 4k elements, the advantage disappears since RDMA READ operations can be issued before the previous data items arrive and are queued on the receiving NIC. At that point both approaches will perform very similarly since they are both network bound, given the amount of data transferred. Since most applications use smaller data sizes, we conclude that the \textbf{SA} offers an important advantage for this type of access. It is also interesting when combined with filtering operators, a very common combination in query processing. 

\input{graphs/filters}

\subsection{Matrix Transposition}

A more involved strided access is to automatically transpose a matrix, a common operation in machine learning and HPC. The transformation can be done easily in the dynamic regions, where the data is first read using the \textbf{SA} operator into the on-chip memory (BRAM, UltraRAM) with fast random-access performance and then transferred over the network in the requested order. As a baseline for comparison we use a two-sided RDMA verb and involve the CPU to rearrange the matrix prior to sending it as it would be done in remote memory.

%\input{graphs/mtrx2}

We implement a 2D matrix transpose \textbf{MT} operator giving either the row-major or column-major view to the client. The interface has the following parameters: 1) \textit{Rows}, the number of rows in the matrix, 2) \textit{Columns}, the number of columns,  4) \textit{Order}, the requested ordering (row vs column). Figure \ref{fig:mtrx} compares the time to retrieve a transposed matrix for different matrix sizes between Farview and a two-sided RDMA operation where the transposition is done on the CPU. The results deliver insights on the CPU overhead caused by operators. As the figure shows, matrix transposition on a CPU is far more expensive than using smart disaggregated memory. %The \textbf{MT} operator is network bound at the sizes tested. 



\section{Smart Filtering}

We now discuss filtering views, i.e., views that transfer only the required data by selecting before transmission. Such views reduce the network bandwidth required and, in certain system configurations (as shown with selection), can lead to better memory performance. The filtering is done in Farview directly on the passing data streams and, besides the resource utilization, does not incur any other significant overhead beyond a slight added latency to receiving the first bit.

\subsection{Reducing Precision}

%\input{graphs/reduced_prec}

Machine learning methods using lower precision input data are gaining traction as they reduce the overhead in training and incur less data movement \cite{Ce17,Blott20}. We use Farview to seamlessly provide different precision views to retrieve data at arbitrary precision levels. Unlike striding, the data is read sequentially and only the required bits for a given precision are kept and sent over the network. By doing this, Farview is able to maximize the available memory bandwidth and achieve a lower total latency compared to the commercial NIC.

%To explore how to combine the idea with smart disaggregated memory, we have borrowed a recently developed multi-resolution data representation for in-memory data, ML-Weaving \cite{Wang2019}, and use Farview to provide an operator that can retrieve the data at arbitrary precision levels. Unlike striding, where we read entire data items separated by a given offset, the data in this case is read sequentially. However, the bits next to each other correspond each to a different data item so the data must be reconstructed if more than 1 bit precision is needed.  We have implemented the reduced precision (\textbf{RP}) operator to enable this functionality in Farview.

The \textbf{RP} operator exposes the following interface: 1) \textit{Tuples}, the number of data items to fetch, 2) \textit{Precision}, the requested precision. Figure \ref{fig:reduced_prec} shows the total latency reading 1000 elements at different precision levels in Farview, compared to using the commercial NIC. The data is stored in an 8 byte format. When reading the full precision (8 byte), the cNIC offers higher performance, matching the results in the microbenchmarks. As the data is read at reduced precision, the ability of the Farview to efficiently exploit the remote memory bandwidth becomes apparent, while for the conventional NIC, reduced precision does not result in any significant advantage over reading the full precision data.

\subsection{Selection}

%\input{graphs/lat_selection}

\input{graphs/transform}

Farview makes it very easy to apply filtering directly on the data streams as they are read from memory. The predicates for filtering can vary; in our example we implement a non-equality based selection operator (\textbf{SL}) similar to that found in many databases and data processing systems. The data is retrieved, evaluated, and transferred only if the predicate is true. We combine this operator with the striding one to have an even more realistic implementation of a memory traversal with filtering also demonstrating one of the ways operators can be chained in Farview. 

Figure \ref{fig:lat_selection} shows the latency comparison between a baseline consisting of one-sided RDMA read where the complete data set is read (without selection) and the read with the \textbf{SL} operator for a number of different transfer sizes. We generate an unsigned 64-bit uniformly distributed data set with value ranges between 0 and 1024. For the selection criteria we filter the data higher than 512. We then increase the comparison threshold, thus increasing the selectivity of the filter (50->25\%). The results show how filtering speeds up retrieval when compared to bringing the data from the disaggregated memory to be filtered locally.

\subsection{Regular Expression Matching}

Farview provides increasing advantages as the computational complexity of the filtering increases. To demonstrate this, we integrate an open source regular expression library (\textbf{RX}) for FPGAs \cite{regex17} into Farview and use it to read strings from the disaggregated memory. Data is retrieved from the remote node only when it matches the regular expression. The operator implements regular expression query acceleration with multiple parallel engines, instantiated in the FPGA. Unlike software solutions, the performance of the operator is dominated by the length of the string and does not depend on the complexity of the regular expression. We compare the average latency of a single string match for different string sizes between Farview and two-sided RDMA verbs where the matching is executed on the CPU, demonstrating once more the advantages of smart disaggregated memory over remote memory that relies on the remote CPU for processing. Figure \ref{fig:regex_comb} shows this comparison. For now, the focus is on the non-chained series in the figure (Farview vs two-sided). In Section \ref{sec:encryption} we will provide further example of this operator in a more complex case, chained with the encryption and decryption operators.

\section{Smart Transformations}

We conclude the exploration of smart disaggregated memory with views that manipulate the data, thereby implementing near data processing capabilities. We present two  operators: calculating basic statistics on data being read (used in databases \cite{Histograms14}) and encryption/decryption. 

%A variety of data transformations can be realized with Farview without incurring any substantial performance penalties. Stateful algorithms like running average, prefix sums can be piggybacked directly onto the data streams. Similarly, data sketching algorithms, like count min, approximate a certain portion of the large data sets and can easily sustain the full network throughput. Stateless non-blocking algorithms can be easily implemented as well, like AES and Chacha encryption, and provide a simple means to secure the data in the far memory without incurring added latency when data is read. 

\subsection{Basic statistics on data streams}

%\input{graphs/lat_average}

In many applications, data is often read just to perform a simple calculation over it (e.g., sum or average). Such operations can be implemented in smart disaggregated memory with computation done as the data is read from memory. There are two ways to use the results. Some applications might be interested in the aggregation, others could be interested in the raw data as well as a summary of the data through such aggregations \cite{Histograms14}. In the latter case, the result of the aggregation can be appended at the end of the data being read.

To test the idea, we have implemented a running average operator, \textbf{RA} computing the average of a stream of numbers read from memory. In Figure \ref{fig:average} we measure the time to read a growing amount of data (64-bit) and compute its average on disaggregated memory vs fetching the data with the average calculated on the CPU using two-sided RDMA operations.

The differences become substantial as the data grows, demonstrating that even simple operations can have a significant impact, especially if the application is interested only in the average. These operators show that, in addition to filtering and addressing, smart disaggregated memory can be an effective platform for near memory processing. 
% instead of the whole data
%, even if only simple transformations are supported. 

%can be a good platform to implement near memory processing even if only simple transformations are supported. 

\subsection{Encryption/Decryption}
\label{sec:encryption}

%\input{graphs/encryption_sbs}
%\input{graphs/thr_aes}
%\input{graphs/encryption_lat}
%\input{graphs/regex_comb}

%\input{graphs/lat_chacha}

A key concern for both remote memory and smart disaggregated memory is the need for data encryption \cite{GoogleFarMemory19}. Farview implements encryption so that the data is treated similarly to Microsoft's Cypherbase \cite{Cypherbase15}, where a database stores only encrypted data but can still answer queries over such data by using an FPGA as a trusted module. 

%To demonstrate the feasibility of encryption in Farview, 
We have implemented encryption as an operator using 128-bit AES in counter mode. Since the AES module is fully parallelized and pipelined, it can operate at full network bandwidth. This means that no throughput penalty is paid when this operator is applied on the stream, incurring negligible overhead in latency. This can be seen in Figure \ref{fig:encryption_thr}, where the data is read through RDMA and decrypted in addition, before being sent. As the graph shows, there is no performance penalty, indicating that encryption/decryption can be easily combined with all the previous operators we have discussed to allow applications to encrypt the data residing in the disaggregated memory and decrypt it before sending it or for processing purposes. The comparison to two-sided RDMA implementation is also made in Figure \ref{fig:encryption_lat}. The significant overhead imposed by the same encryption in counter mode done on a remote CPU with \textit{OpenSSL} \cite{openssl} library can be seen.

To provide a more complex example of encryption integration and operator chaining, we implement an operator that decrypts the encrypted strings, matches them against the given regular expression and then encrypts the results prior to sending them over the network. The average latencies of these operations for a single string of different sizes are shown in Figure \ref{fig:regex_comb} (chained operators). The overhead of both the encryption and decryption is negligible in Farview, compared to the case where only regular expression matching is done.

%The benefit of having multiple concurrent regions is the ability to dynamically share the available network bandwidth between them, especially when multiple operators have high operational intensity. Here, the compute bound nature allows processing to proceed in multiple regions at full throughput as the available network bandwidth is sufficient. We implement the ChaCha (\textbf{CC}) encryption algorithm. The operator consumes the plain text and produces a cipher at a maximum rate of \textasciitilde 1.45 GBps. The operator is thus compute bound and the total network bandwidth is more than sufficient to support the operation at full throughput for a number of these operators running in parallel. Figure \ref{fig:chacha} shows the total execution time for different transfer sizes when processing is distributed in multiple concurrent regions vs the case where the processing is confined to only a single region.

%\subsection{Inference}

%\input{graphs/dtrees}

%\textcolor{red}{We need to be careful to be different than Coyote}
%As an example of a more complex operator we implement decision trees (\textbf{DT}), one of the most popular supervised machine learning algorithms. They are used for a range of different machine learning tasks. We integrate Gradient Boosting decision trees, the most common form. For testing, the tree model is first generated and placed in the disaggregated memory. At that point the operator can do inference on any passing data streams. 

%We run the tests for the various tuple sizes where each tuple is made of 25 features, 4 bytes each. If higher throughput is required, multiple parallel instantiations of the decision tree engines can be instantiated. When this is the case, the inference can compeletely be hidden behind memory transfers. Thus, the results of the inference can be sent with the accompanying data in the same fahsion as was the case with far simpler running average and prefix sum operators.







==> chapters/chapters_asplos/introduction.tex <==
\section{Introduction}

As performance requirements become more demanding and the amount of data processed increases, %the overhead of moving data has become a serious bottleneck. Combined with the separation of compute and storage prevalent in all major cloud deployments (e.g., Amazon, MS Azure, Google), it has led to 
there has been a widespread adoption of in-memory computing. As a result, there is a growing interest in ways to expand memory systems: near memory processing \cite{OracleM716,Accorda-19}, in-memory processing \cite{PIM18,InMemoryP18}, far or remote memory \cite{RemoteMemory17,Farmemory19,FarMemory20}, far persistent memory \cite{AsymNVM20}, disaggregated memory \cite{Blades09,gao16,Legos18,Dis12}, smart or active memory \cite{Caribou17}, etc. 
These developments are occurring at a time when hardware is evolving quickly, with architectures departing from the Von Neumann model and through innovations in networking like RDMA, software defined networks, or smart NICs. %that provide alternative access channels and create the possibility to design systems in a fundamentally different way. These 
These changes are transforming the conventional notion of memory, which is no longer just a load/store device. 

%For instance, several studies exist using remote memory as a swapping device for local memory either using standard I/O interfaces \cite{Blades09,Dis12} or, in more modern versions, RDMA \cite{FarMemory20}. NVM, being a combination of memory and storage, is tackled through even higher level interfaces such as file systems \cite{Octopus17}, Key-Value-Stores (KVS) \cite{Caribou17,FlatStore20}, or as a pool of persistent memory out of the NVMs attached to servers \cite{AsymNVM20}. Common to some of these more recent efforts is the use of RDMA \cite{AsymNVM20,FarMemory20} which is increasingly being also supported by smart NICs \cite{Lynx20,Strom20,KVdirect}, an aspect we explore in this paper as it can play a role in reducing the overhead of using memory across the network. 

Motivated by recent results indicating that DRAM capacity has become a major limitation in cloud computing due to the growth of in-memory data analytic applications  \cite{GoogleFarMemory19}, in this paper we focus on \textit{smart} disaggregated memory in the form of network attached DRAM through a smart NIC. This is an unexplored combination that, as we will show in the paper, offers unique advantages over existing solutions. In fact, some of the limitations of disaggregated memory raised in the past (e.g., why attaching an expensive, fast memory to a comparatively slow network) can be addressed through advances in networking (RDMA offering microseconds latency and more powerful interfaces) and smart NICs allowing to move computation close to the memory and, thus, potentially compensate for the network overhead. %Using DRAM, with it slow latency and high bandwidth characteristics, helps support multiple users concurrently and provides the necessary capacity to process the data near the memory before being sent to the application without actually affecting latency in a significant manner. 

Unlike previous approaches using, e.g., a paging interface to memory located elsewhere \cite{Blades09,Dis12,FarMemory20}, we opt for a more flexible design enabling applications a better control of bulk data transfers. Our approach is based on the notion of \textit{logical views}, a concept we borrow from relational databases. Views are used in databases to obtain logical data independence. Instead of enforcing a unique data schema on all applications, views allow different users to see the data organized in different ways even if the logical (schema) and physical representation is the same for everybody. We believe the notion of views over disaggregated DRAM dynamically tailored to the applications through a smart NIC offers significant advantages.   

To implement, test, and evaluate these ideas, we have developed \textit{Farview} (FV), a novel, open source research platform for prototyping disaggregated memory. Farview is based on a smart NIC implemented on an FPGA with the FPGA having access to sufficient local memory (DRAM) to act as a disaggregated, network attached memory module. %The FPGA is connected to a server through PCIe so that it can also be used as a platform for implementing remote memory (memory of a different machine that is accessible through the network). 
The smart NIC is built on top of our own FPGA shell, enabling the FPGA to be partitioned into logic regions that can be dynamically reconfigured to deploy different near-memory processing functionality. These regions can all independently and concurrently access the local memory on the FPGA and communicate through RDMA. 
The smart NIC supports RoCE v2 at 100 Gbps in the form of an open source RDMA stack, enabling us to optimize interaction between network and memory. %The design of Farview is also suitable to compare remote memory (shared memory attached to a computer) with disaggregated memory (sahred memory that is not part of a computing node).

%While we focus on a number of potential designs, the lessons learned apply to many other architectures being considered for improving the memory stack. In particular, with very few exceptions \cite{Farmemory19}, most of the work being done around memories does not discuss in any detail how the new possibilities offered affect the memory abstraction and its interface. In other words, in spite of the performance gains often demonstrated, in many recent results it is not obvious at all how an application would actually use the new features, let alone several applications operating concurrently. In this paper we explore in detail how disaggregated memory could be used and discuss the practical implications of such use cases on both performance as well as the way applications would treat memory. The focus is not so much on showing that a given use case is better than some baseline. Instead, we analyze where the performance gains come from and explore the flexibility offered by Farview through the implementation of \textit{views} over the data in the relational database sense: the data can be seen by different applications in a different manner, regardless of how it is actually represented in memory. 

%The study is enabled by a novel, open source memory prototyping system, Farview, that allows the exploration and comparison of alternative disaggregated memory configurations.

In this paper we focus on read-only workloads involving bulk data transfers as those play a big role in in-memory data analytics \cite{GoogleFarMemory19}. Our use cases include  applications from data science, data processing, high performance computing, and machine learning. For these applications, we explore how to use smart disaggregated memory using three categories of views over the data: (1) \textit{addressing} operators providing sophisticated forms of addressing and accessing memory; (2) \textit{filtering} operators that read data only matching a given predicate; and (3) \textit{transformations} that actually perform data processing in-situ before or in lieu of sending the data. 

%Among the first category are views that enhance the standard memory interface for loading data. We first study pointer based traversals of data structures such as skip lists and hash tables. We then look into accesses to data collections using a fixed stride and matrix transposition. Among the second category are views filtering the data being read. We implement selection where only data is transferred matching a given predicate and reading the same data at different numeric resolution levels. Finally, the third category involves the ability to compute over the data while it is being sent or instead of sending it.  We demonstrate the computation of prefix sum, running averages, aggregation, and data sketches over the data being read. 

The contributions of this paper are: 
a proposal for memory views, an interface for smart disaggregated memory that raises the level of abstraction from traditional memory systems; 
an open source platform, Farview, for studying novel network-attached memory systems;
using Farview, the implementation of eight memory-side operators in three categories of views;
and a comparative evaluation of memory views vs. one- and two-sided implementations on a commercial smart NIC.

% KK note: we aren't even close to comprehensive.
% With these examples, we provide a comprehensive perspective on disaggregated memory and its potential when extended with RDMA and smart NICs. The contributions of the paper, in addition to these examples and the detailed study of smart disaggregated memory, include the open source platform  we use for the evaluation, Farview, that will play an important role in studying future network attached memory systems. 


==> chapters/chapters_asplos/system.tex <==
\section{Farview}

Farview is a platform for prototyping smart disaggregated memory that exposes an API of views over the stored data providing complex addressing modes, data filtering, and data transformations. Farview is implemented in an FPGA-based smart NIC by extending RDMA one-sided verbs to raise the level of abstraction provided by the memory. Farview is open source and has been designed for flexibility and exploration rather than aiming for the peak efficiency that might be possible with a custom hardware implementation. In the following sections, we describe the views API and provide an overview of the Farview architecture and its implementation.

%Farview is an open source platform built for prototyping disaggregated memory. It %is not intended as an implementation of disaggregated memory since it 
%has been designed for flexibility and exploration rather than efficiency. Consequently, in what follows we focus on the novel features of Farview and those relevant to disaggregated memory. %For features that are common on FPGA based systems and have been discussed elsewhere, we refer to related work. 

\subsection{Views API}

Farview exposes the data stored on smart disaggregated memory through a set of views that present data to users in logical representations rather than in the way the data is physically stored. In Farview, these views are implemented by a set of \textit{operators}. Farview currently implements three categories of views: (1) \textit{addressing} operators supporting sophisticated forms of addressing and memory access; (2) \textit{filtering} operators returning only the data matching a given predicate; and (3) \textit{transformation} operators that perform data processing in-situ before or in lieu of sending the data. We demonstrate eight operators in these categories, including a hash table with indirect addressing, strided memory traversals, matrix transposition, reduced precision retrieval, predicate-based selection, regular expression matching, basic statistics on data streams, and encryption/decryption.

Farview exposes a simple high level API to the clients. Upon the establishment of the connection to the remote back-end node, the clients are provided with the created object representing it (\textit{QPair}). This object holds all the necessary information for a specific connection and is passed to any of the subsequent Farview methods (see Section~\ref{subsection:net_stack}). The available back-end operators providing a variety of views can be dynamically loaded and exchanged. This swap is in the order milliseconds, depending on the size of the operator (see Section~\ref{subsection:reconfig}). The following function is used for this purpose:

\begin{lstlisting}
bool loadView(QPair *qp, FView *fv);
\end{lstlisting}

The memory in the back-end can be allocated with the following allocation functions:

\begin{lstlisting}
uint64_t* allocMem(QPair* qp, uint64_t size);
void freeMem(QPair *qp, uint64_t* mem);
\end{lstlisting}

The actual read and write RDMA and Farview requests are sent with the following functions:

\begin{lstlisting}
void rdmaRead(QPair* qp, uint64_t src_offs, uint64_t dst_offs, uint64_t size);
void rdmaWrite(QPair* qp, uint64_t src_offs, uint64_t dst_offs, uint64_t size);
void farView(QPair* qp, uint64_t *params, uint64_t size);
\end{lstlisting}

The first two correspond to standard RDMA read/write requests. The third, the \textit{farView} function, corresponds to a specialized RDMA verb (based on RDMA Write) that invokes a particular disaggregated memory operator(s) with an arbitrary parameter set specific to each view. This generic function is used as the basis for building additional interfaces supporting the specific operators. As an example, the function prototype for the strided access (\textbf{SA}) operator (built on top) is as follows: 

\begin{lstlisting}
void farStride(QPair* qp, uint64_t src_offs, uint64_t dst_offs, uint64_t size, uint64_t count, uint64_t stride);
\end{lstlisting}

\subsection{System Overview}

\begin{figure}[t]
\centering
\includegraphics[width=0.85\columnwidth]{figures/system2.pdf}
\caption{Farview prototyping platform }
\label{fig:system}
\end{figure}

Prototyping smart disaggregated memory requires several components, including DRAM, memory controllers, a network stack, a mechanism to support concurrent access to the memory, and a smart NIC capable of running operators acting either on the memory accesses or the data being transferred. Modern FPGAs, which offer flexibility in design, are equipped with a growing amount of local FPGA-attached memory \cite{u250} (e.g., up to 512 GB on some experimental systems~\cite{Enzian20}). We leverage this design flexibility and implement Farview on an FPGA, as shown in Figure \ref{fig:system}. For ease of control, programming, and management, the prototype FPGA card is coupled to a host computer over a PCIe link. Section~\ref{sec:eval} provides more details of our experimental setup.
%Farview leverages this flexibility to implements these components on an FPGA, 
%Modern FPGAs are usually equipped with a growing amount of local, FPGA attached memory \cite{u250} and some experimental systems have announced up to 512 GB of local memory on the FPGA \cite{Enzian20}. This memory provides better performance than memory attached over PCIe. Multiple banks are usually present offering additional parallelization potential, a crucial advantage in the type of workloads targeted by Farview.
%(\todo this is one of the aspects that would be different in a real, disaggregated implementation). As it is common in such designs (e.g., Intel's HARP or Amazon F1 instances), Farview contains a fixed region where we deploy the Farview infrastructure (network stack, memory controllers, etc.) and a reconfigurable region where we deploy the operators.

To manage concurrent connection flows, Farview uses multiple \textit{dynamic regions} on the FPGA, each implementing a view operator. These regions are dynamically reconfigurable, the logic deployed in them can be changed at run time without having to reconfigure the whole FPGA. These dynamic regions are part of the operator stack. They are placed between the network stack and the memory stack and are provided with standard interfaces to both, so that programmers only need to focus on the application logic and not on the connectivity. 

%This logic is what is used to turn the disaggregated memory into \textit{smart} disaggregated memory by implementing the memory access operators.

The network stack manages all external connections and RDMA requests. It identifies flows using \textit{queue-pairs}, information that is used internally as well as to route the flow of requests and data through Farview accordingly. For networking we use an open source RoCE v2, 100 Gbs network stack \cite{Strom20} that we have adapted and extended. Section~\ref{subsection:net_stack} describes this stack in more detail.

The memory stack houses the memory management unit (MMU) which handles all address translations to dynamically allocated memory on the FPGA, allowing applications to use one or more of the available memory channels. It provides the necessary arbitration as well as isolation between concurrent accesses by different applications.
%It provides the necessary arbitration and, especially, isolation between different concurrent accesses since the goal is to implement a dynamic memory pool used concurrently by different applications. 
Section~\ref{subsection:mem_stack} describes this stack in more detail. %Although not relevant for the purposes of this paper, the MMU provides access to both the local and the host memory. 

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figures/region2.pdf}
\caption{Single dynamic region with its interfaces}
\label{fig:region}
\end{figure}

Figure \ref{fig:region} illustrates the operation of a single dynamic region. As described in the previous section, the Farview API provides both the standard one-sided RDMA read/write commands to read or write data from/to memory and a Farview verb, implemented as a one-sided operation that invokes the loaded operator over the read or write data stream. A request is processed as follows. First, the request's virtual address and transfer length parameters are forwarded to the memory controller (the blue path in Figure \ref{fig:region}). If the request is a simple RDMA read/write request, it contains no additional parameters. If the request is a Farview verb, it carries a number of operator-specific parameters (green path). Control of the memory access patterns for operators takes place in the Farview request handler, while the data processing occurs along the read/write RDMA data paths. Responses to these requests are sent through the RDMA stack (red path). With this architecture, operators can dynamically control and influence the size of the response data transfers. This enables the implementation of filtering, for instance, where the size of the filtered data is unknown prior to the processing. The direct data streams between memory controller and network are sized to saturate the available bandwidth and to provide optimal performance.

%Farview's logic inside the FPGA consists of the network and memory stacks plus the application regions. For the network stack, we extend and adapt STROM, an open source  RoCE v2, 100 Gbs implementation \cite{sidler2019innetworkdataprocessing} available in high level synthesis (HLS) and that has been used to implement smart NIC supported RDMA across machines in distributed applications such as Key-Value Stores. It implements RPC semantics that are invoked through one-sided RDMA operations. 

%The two novel aspects in the design of Farview are the application regions and the memory controllers. 

%The application stack provides an FPGA \textit{hardware partition} layer based on spatial and temporal sharing that enables the execution of different concurrent applications. The application stack is divided into separate virtual FPGA regions which can be independently loaded with custom operators developed in any of the most commonly used HDL or HLS programming languages. These operators are placed directly on the path to/from memory of the incoming or outgoing network streams so that they can operate directly on them. 

\subsection{Network Stack}
\label{subsection:net_stack}

The network stack we use implements a reliable RDMA connection protocol. We extend the original stack with support for out-of-order execution at the granularity of single network packets since this is an important feature in a disaggregated memory setting. The original stack implements regular one-sided InfiniBand verbs: RDMA write and RDMA read. Similar to other remote memory systems based on RDMA, (e.g., \cite{AsymNVM20}), we add an additional Farview one-sided verb to control the  operators. It includes a number of additional parameters containing the necessary signals to the disaggregated memory on how to access data (addressing operators), how to process it (filtering operators), or how to change it (transformation operators). The network stack manages connections, buffers, and keeps the necessary state while remaining highly customizable so that it can support further extension to how disaggregated memory operates. It exposes a defined set of streams corresponding to each connection flow and each dynamic region.

In RDMA, the information describing a single node to node connection or RDMA flow is associated with a \textit{queue pair}. The queue-pairs contain unique identifiers which are used to differentiate the flows and to provide the isolation through a series of hardware arbiters. Upon connection establishment, each flow and its corresponding queue pair gets associated to one of the dynamic regions. The operator (or operators) corresponding to the specialized requested view can be loaded into the dynamic region, and the flow is then ready to be processed. Queue pairs are also used to keep track of the dynamically allocated  memory locations used in the RDMA requests between remote nodes. This allocated memory can be shared between different queue-pairs.  %The information in the queue pairs is exchanged prior to the operation and this can be done over the regular TCP/IP network\textcolor{red}{Am I calling this correct?}.

%The open-source RoCE v2 network stack supports  RC (\textit{Reliable Connection}) protocol and the execution of RDMA operations. The stack uses the board's 100G Ethernet connection and is able to process packets bi-directionally at 100Gbps. It implements the regular one-sided InfiniBand verbs: RDMA WRITE and RDMA READ.  The incoming and outgoing network channels are fully decoupled enabling processing at full line rate. All the necessary states and queue pair connection details between the remote nodes are stored locally. These are stored in the on-chip memory along with the necessary information on allocated memory resources and the assigned dynamic processing regions where the streams can be routed. 

%The network processing of the packets starts with the extraction of IP and UDP headers. Further information necessary for processing of the packets is contained in additional base and extended transport headers. The BTH (\textit{Base Transport Header}) supplies the op code, the target queue pair number with which the local state is accessed and the PSN (Package Sequence Number) used for guaranteeing reliable communication. At this point all the necessary external routing information is read and provided. The RETH (\textit{RDMA Extended Transport Header}) provides the memory access descriptors. These descriptors hold the user space virtual addresses pointing to the allocated memory buffers, previously exchanged between the queue pair nodes, enabling the remote memory access through the MMU. Before the actual memory accesses, the Farview routes the network streams to the appropriate virtual FPGA regions, loaded with custom user kernels and permitting direct in the flow processing. The extension to the stack brings the RPC READ and WRITE verbs. This allows remote passing of the parameters and the creation of custom interfaces responsible for the interaction with deployed user kernels. These kernels can perform direct transformation during the memory access operations.

%Both RDMA READ and RDMA WRITE verbs provide little room for transferring additional information and parameters needed for remote procedure calls. To enable this, we implement additional RPC READ and WRITE verbs which allow remote users to issue the RPC requests. The RPC READ first sends a request embodied in the added transport header RPCETH (RPC Extended Transport Header). This header contains information similar to RETH, but provides an additional field containing arbitrary parameters which are consumed by the target user kernel doing the processing. The size of this header is a compile time parameter and can differ from RETH. The exact response and behaviour to these parameters is decided by the implemented kernel. The RPC response and the accompanying data is then supplied via RDMA WRITE verb in the opposite direction. The RPC WRITE can be used to process data transparently on the incoming streams.

%The growing FPGA sizes and high performance 100G connection open the space for concurrent processing where multiple deployed applications and flows can run side by side and share the available bandwidth. This is supported by the virtualization layer present in the Farview. The layer permits a relatively large number of parallel spatially and temporally shared dynamic regions in the FPGA loaded with custom user kernels. All the network packets can be processed in the out-of-order fashion from multiple FPGA regions. This allows the RDMA stack to multiplex multiple application streams and leads to better optimisation of the network bandwidth. The fair-sharing between different user regions is imposed by the round robin arbitration implemented in hardware arbiters.

%The virtual FPGA regions are tied to the queue pairs. Each queue pair in the RDMA state table is assigned to one or more specific region IDs. Each network RDMA transfer is initiated with the appropriate command. This command holds the requested op code, memory descriptor and in the case of RPC, parameters necessary for memory accesses and processing in the kernels. The command can also be issued from the virtual FPGA regions directly. Additionally, the region ID and operator ID are contained. The region ID routes the command to the appropriate virtual region, whilst the operator ID is used to compare the loaded region operator to the one requested by the RDMA command. If the IDs differ, the partial reconfiguration can be initiated and target operator can be loaded with the partial bitstream containing it.

\subsection{Memory Stack}
\label{subsection:mem_stack}

The central part of the memory stack is the memory management unit (MMU) responsible for all memory address translations to a shared dynamically allocated memory. It propagates all memory requests and subsequent data. It supports the issuing of multiple outstanding requests and has fully decoupled read and write channels. It provides parallel interfaces, isolation and protection for all the requests stemming from different dynamic regions with a set of arbitrators, crossbars and dedicated credit-based queues.

The MMU contains a translation lookaside buffer (TLB) implemented with the fast on-chip memory. In Farview, it is software loaded from the host CPU and it holds all virtual to physical address mappings for the dynamic regions. The memory allocation is dynamic and is handled by the Linux kernel driver module with a pool allocator. This allocation is invoked by the client with the API functions. In a commercial implementation, this can be done either by a small external CPU or in the same FPGA with one of the \textit{softcore} CPUs directly implemented in the FPGA fabric \cite{microblaze}.

Farview's MMU supports naturally aligned 2 MB pages. This greatly reduces the coverage problem of smaller pages (an observation shared with the design of Optimus \cite{HyperFPGA20}). Farview's MMU also abstracts the memory channels and banks. It provides a transparent abstraction for DRAM accesses that maximizes the available DRAM bandwidth by aggregating the bandwidth from multiple channels (if present). It also partitions data automatically across the banks to enable such functionality for write requests that automatically have their data spread across banks. Read operations over partitioned buffers only see an increase in the available bandwidth. 

%Instead of regular 4kB page size, typical in most of the host MMUs, the Farview supports naturally aligned 2MB pages, the access to which is provided by the hugepage Linux library.

%As well as entries for the FPGA attached DRAM, the TLB can also contain mappings that refer to memory over the PCIe (e.g., Non-Volatile Memory or HighBandwidth Memory). A flag bit in the TLB entry specifies whether the virtual address points to a location on the host or on the FPGA. This flag thus determines the correct routing for the requests and subsequent data. The memory requests that leave the MMU are then processed by the appropriate DMA engine. 

\subsection{Operator Stack}
\label{subsection:oprator_stack}

The operators deployed in the dynamic regions are written against the interfaces exposed by the Farview's network and memory stacks. They are portable across Farview deployments, regardless of the underlying FPGA. They can be written in common hardware description languages like VHDL or Verilog,  as well as in high level synthesis tools such as Vivado HLS. 
Within the regions, programmers can use a number of available hardware resources, such as dedicated on-chip memory with very low random access latency (BRAM, URAM) or specialized DSP blocks for floating-point computation. The only restriction is to conform to the provided set of interfaces when accessing memory and interacting with the network since each dynamic region is placed as a bump-in-the-wire where it can process the incoming and outgoing data directly.

The operator stack is where this smart logic attached to each connection flow to/from memory is deployed. It is implemented as a collection of pre-defined dynamic regions where logic can be deployed at run time and swapped on-the-fly without affecting the integrity and operation of the system or other operators. These regions and their access to memory are isolated from each other (see Section~\ref{subsection:mem_stack}). 
Such functionality is typically not available in commercial systems, but very often studied in the literature, e.g.,  \cite{AmorphOS,HyperFPGA20,VirtualFPGA20}. Compared to existing FPGA frameworks, in Farview the regions have to be connected to the network and memory stacks, reducing the degrees of freedom in placement and sizing. Linking dynamic regions to an actual network stack is different from linking them to the Ethernet (PHY and MAC) connector(s) available in the FPGA. 
%\todo\textit{We might even go for the removal of this part completely.} 
For instance AmorphOS \cite{AmorphOS} does not consider the network at all, neither as a physical connector nor as a network stack. Optimus \cite{HyperFPGA20} and ViTAL \cite{VirtualFPGA20} do virtualize the Ethernet connector but only at the physical level, %The latter just connects the regions to the Ethernet interface without any arbitration of the access to that interface 
as this is enough to communicate across FPGAs using point-to-point links in a ring topology without going through a network switch \cite{VirtualFPGA20}. 

Due to the spatial architecture of FPGAs, elements with a fixed location like the memory controller, and especially large ones like the network stack, pose significant challenges in the design. 
%In Farview the dynamic regions need to be connected to logical elements (RDMA queue pairs) rather than to a given hardware module and these connections need to be mapped rather than \textit{wired} as they can change at run time. %Additional differences between existing systems and Farview is that 
Farview always places logic between the RDMA stack and the memory controller as the only purpose of the system is to implement a smart NIC rather than arbitrary functionality. The management infrastructures in Farview have to cope with line rates of 100 Gbps, something that requires 512 bit wide buses \cite{Strom20,Limago19} and introduces quite a few restrictions on the placement of the regions and the ability to give them arbitrary sizes. Hence the choice of pre-defined regions. 

%A schematic of a single dynamic region and the corresponding interfaces is shown in Figure \ref{fig:region}. Within each dynamic region, signals are split between request commands (either RDMA READ/WRITE or a specialized verb) and RDMA data streams. All of them provide a simple, high performance, handshaking protocol commonly found in systems of this type \cite{Strom20}. The rest of the dynamic region is quite flexible and can be used in a variety of ways. 

%In Figure \ref{fig:region} we show an example where, similar to the ones used in the filtering operators, request processing (potentially involving non sequential accesses) and data processing (matching data items against a predicate) are decoupled to maximize throughput. %Generic handler and state keeping modules can be further adapted to the specific needs.

%If dynamic reconfiguration is triggered, the pre-validated partial bitstreams are streamed from the host memory, via PCIe. These streams are then redirected into the ICAP unit. The ICAP is a hardware primitive used to receive the partial bitstreams and reconfigure portions of the FPGA logic. As only one dynamic region can be reconfigured at a time, locking is employed by the Farview driver module. By using a high performance data stream we are able to fully saturate the maximum supported bandwidth of the ICAP which equals to ~800 MB/s. In comparison, framework like SDAccel \ref{} achieves only 19 MB/s of reconfiguration throughput. The partial reconfiguration can be initiated by the RPC call. The request holds the operator ID which is used for comparison with the currently loaded region. If these do not match, partial reconfiguration can be executed. However, the overhead of the reconfiguration is still significant and it is in the order of the milliseconds, depending on the size of the region. For this reason, the reconfiguration can also be initiated from the local CPU. This can occur during the queue pair exchange between the remote and local nodes. The remote node can signal to the host exactly which operators it needs for the following transfers. The reconfiguration provides vast flexibility as it allows large number of operators and transformations to be supported. 

==> chapters/earlier_versions/abstract-2021-02-18.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
Cloud deployments disaggregate storage from compute, providing more flexibility
to both the storage and compute layers.
%The added latency caused by the network in between is often compensated with
%near-data processing (most storage layers support some form of data processing
%at the storage layer) and/or through caching layers. 
In this paper, we explore disaggregation by taking it one step further and applying it to memory (DRAM).
Disaggregated memory offers network attached DRAM as a way to decouple memory
from CPU. In the context of databases,
such a design offers significant advantages in terms of making a larger main
memory capacity available as a central pool to a collection of smaller processing nodes.
% KK: suggest clarifying what's unsolved/new, so it's more obvious what problem we're solving
To explore these possibilities, we have implemented \textit{Farview}, a disaggregated memory solution for databases 
operating as a remote buffer cache with operator offloading capabilities. We prototype Farview as an FPGA-based smart NIC that makes DRAM available as a disaggregated, network attached memory module capable of performing data processing at line rate over data streams to/from disaggregated memory.
%To reduce latency, we use RDMA between the disaggregated memory and
%the computing nodes, with the disaggregated memory using a smart NIC to enable
%data processing at line rate directly over the data streams to/from memory.
% KK: better from my perspective: We present \textit{Farview}, a smart disaggregated memory that acts as a remote database buffer cache with operator offloading capabilities. 
% KK: still need to work in somewhere that the Farview prototype platform is open source. I believe that RDMA is ubiquitous enough that we don't need to say that we're using RDMA to reduce latency over TCP/IP.
%
% In addition, we implement support for the equivalent of \textit{views} over
% the data in that the disaggregated memory can pre-process the data using
% different relational operators before sending it to the computing node. In this way,
Farview supports query offloading and view materialization using operators
such as selection, projection, aggregation, regular expression matching, as well
as compression and encryption. 
% KK 2/18/21: "query offloading" or "operator offloading"? and aren't we de-emphasizing view materialization?
In this paper we focus on analytical queries and
demonstrate the viability of the idea through an extensive experimental
evaluation of Farview under different workloads. Farview is competitive to a
local buffer cache solution for all the workloads and outperforms it in a number of cases, proving that a smart disaggregated memory can
be a viable alternative for databases deployed in cloud environments.

%Disaggregated memory has been proposed as a way to scale out the amount of memory available independently of the computing or storage capacity. The idea mirrors the disaggregation of compute and storage in the cloud but takes it a step further and applies it to main memory. %While the idea has been explored in various forms,
%The advent of smart NICs and the adoption of RDMA have opened up new possibilities given the growing demand for in-memory computation. In this paper we explore the design space of disaggregated memory through Farview (FV), an open source prototype for exploring disaggregated memory. We assume the memory is in the form of DRAM, directly attached to the network, and it is not part of a computing node. Access to the memory is through RDMA via a smart NIC that we prototype with an FPGA. Using Farview, we evaluate the trade-offs involved in pushing processing close to the data in disaggregated memory. We show that memory-side processing makes disaggregated memory more suitable for big data workloads (databases, high performance computing, machine learning) through the memory equivalent of relational database views, enabling the same data to be presented to applications in different forms. We discuss possible interfaces to such functionality and evaluate the resulting performance when compared to disaggregated memory without memory-side processing capabilities.
\end{abstract}


==> chapters/earlier_versions/background-2021-02-18.tex <==
\section{Background and related work}

In this section we motivate Farview and discuss related work. The design is based on extensive experience in data center, computer, and processor design \cite{TheMachine1,TheMachine2}, on how hardware is evolving along many dimensions, on the increasing availability of better networking capabilities, and optimization efforts targeting workloads in data analytics and high performance computing. For reasons of space, in here we focus only on the most salient aspects. 
% KK: this para could probably be shortened, if we need space

%\subsection{Databases and data movement}

%Historically, databases have invested significant efforts to reduce the I/O overhead, with I/O being broadly construed. Initially, such an overhead was clearly defined: memory was very limited in capacity and disks were slow. Over time, the bottleneck changed in nature as faster storage became available (SSDs, NVM), memories became larger, caches started becoming an issue, and multicore emerged as the dominant
% KK: not clear whether you mean processor caches (L1/L2/LLC) or buffer cache management. 
%processor design. Yet, the I/O overhead, regardless of whether caused by the disk, the storage, the network, or the caches, remains a major factor in the overall performance. The problem is compounded by three factors: (1) databases induce a lot of data movement, which is known to be a major source of inefficiency in modern computing; (2) the amount of data to be processed keeps growing; and (3) the distributed nature of cloud and data center computing makes the coupling of storage, compute, and memory capacity very problematic from a cost and efficiency point of view. 
% KK: to me, this is the crispest problem statement so far.

%\textbf{Data movement} Optimized query plans typically push down selection and projection operators to filter out the base tables as early as possible. 
%Views are also widely used to tailor the schema and provide logical data independence.
%The declarative nature of SQL makes this a very natural step when producing the query plan or when rewriting a query targeting a view so that it can operate on the base tables. 
%However, the step of going from base tables to the data actually needed by the query is an expensive one. Base tables are fetched from storage as blocks that are placed in a buffer cache in memory. From there, a query thread reads the data and filters it % out 
%to form the input to the rest of the query plan. Often, most of the data is % finally
%dropped because it does not match the query's selection predicate. As more data is involved, the overhead becomes larger. Data movement has been identified as one of the biggest sources of inefficiencies in computer designs \cite{dally2011power,dally2020domain}, making the way databases operate intrinsically problematic from a systems perspective. Of course, many approaches have been proposed to reduce the overhead: data partitioning, zone maps, indexing, using meta-data to retrieve only what is needed, etc. The problem, nevertheless, still remains. The literature on the topic is very extensive and much more than what we can cover here in detail. Sufficient to say that the issue is relevant enough that specialized hardware and architectures are being devised to deal with it (see below). 
% KK: suggest shortening the last few sentences: "Many approaches have been proposed to reduce the overhead (e.g., data partitioning, zone maps...); the literature is too extensive to cover here in detail. The problem, nevertheless, remains, prompting the design of specialized hardware and architectures (see below)."

%\textbf{Data sizes and memory} Relational engines today keep a large part of the data in main memory. Unfortunately, the size of analytical databases keeps growing, so even main-memory databases are confronted with a widening gap between the size of the working set and the DRAM available \cite{Leis-ICDE18}. One way to tackle this issue is to scale-up: provide more DRAM and/or more and faster disks to increase virtual memory capacity \cite{neumann2020umbra}. Such designs have several undesirable consequences: cost (the resulting large servers cannot be easily replicated for, e.g., availability), centralization and inelastic behavior, and exacerbating the data movement problem. 
% KK: not sure what you mean about "and exacerbating the data movement problem" -- NUMA effects?
%Some of the additional problems encountered in scale-up architectures include NUMA effects \cite{NUMA-Shuffling} and load interference \cite{MC-interference}, which in some cases force changes to the way the engine operates. In order to deal with the increasing cost of DRAM, NVM has been introduced as an attractive alternative that, on the one hand, is both cheaper than DRAM and persists data, but on the other hand has larger latency. Database literature has explored how to offload different parts of a DBMS to NVM~\cite{van2019persistent}, build DBMSs on top of NVM \cite{arulraj2019non, arulraj2017build} or use combinations of DRAM, SSD disks and NVM
% KK: "SSD disks" is redundant -- replace with either "SSDs" or "SSDs, HDDs", depending on what the work supports
%to offload different parts of the buffer and storage manager to each storage layer \cite{van2018managing, arulraj2019multi}. 

%\textbf{Distributed data processing} Database engines today tend to be distributed  engines. This is definitely true in the cloud and data centers, where the system architecture favors scale-out designs. %But it is also true in data centers and even smaller deployments due to the possibilities of better matching capacity and load.
%In such distributed settings, we now know that coupling architectural aspects (storage, CPU capacity, memory capacity) to each other is a bad idea, as it leads to inefficiencies due to over-provisioning of one resource when what is needed is a different resource. This is why essentially all cloud designs disaggregate compute from storage. The same arguments used for compute and storage also apply to memory and compute, hence the surge in efforts to develop new architectures that disaggregate memory from compute (see below). For a database engine, memory disaggregation offers an interesting possibility: physically detaching query processing from buffer management can enable a far more elastic design. The buffer cache can reside on a node (or nodes) accessible through the network, with query processing nodes provisioned on demand to run a query by reading the data from the network attached buffer cache. 
% KK: note: this seems similar in spirit to the network attached memory work~\cite{Binnig16}
%Since the processing nodes do not maintain the buffer cache, the memory allocated to them can be smaller. Such nodes can also be ephemeral, since they no longer maintain any part of the engine infrastructure. 
% KK: Q: how does this compare with how Redshift is architected, to support elasticity?
%Needless to say that this has to be done carefully, otherwise the flexibility so gained will come at a high cost in terms of performance and efficiency: inducing even more data movement and higher overheads by involving network data transfers. 
% KK: suggest shortening: "Needless to say..." -> "This redesign must be done carefully, otherwise the flexibility gained will come at a high cost of increased data movement and network data transfer overheads."
%These issues can be addressed by taking advantage of modern hardware.

% KK: This is a more fundamental argument about re-architecting databases to be more elastic, through the use of smart disaggregated memory. I like it, although I don't think we have the experiments to demonstrate elasticity -- that'll have to be our next paper. :) 
% KK: Seems like it would be useful to lead with the DB-specific problem statement (see my comment about crisp problem statement above) and (some of) this vision for how (cloud) DBMSs should be architected.

\subsection{Operator offloading}

The underlying inefficiency mentioned above (reading in an entire base table to discard most of it) occurs at all levels of the memory/storage hierarchy. As a result, many efforts have been devoted to minimize it. Of particular relevance to Farview are efforts that use specialized hardware to enable near-data processing capabilities either in memory or in storage. The argument in favor of such designs is simple: push down selection and projection operators (as well as potentially other operators such as aggregation or even joins where one of the tables is small) to the memory or storage so that the base table is filtered out in-situ and irrelevant data does not need to be moved or sent. Thus, designs exist that add intelligence to local storage so that it can support operator push down and execute SQL operators \cite{Ibex,Your-SQl}, but require a different interface to the storage (since it no longer returns blocks but tuples). Even more ambitious are accelerators embedded in the data path between memory and CPU caches \cite{OracleDAX,Accorda-19} which can filter data as it is read from memory to reduce data movement and cache pollution. These approaches rely on specialized processor architectures and are not widely available. Finally, in the cloud, systems like Amazon's AQUA \cite{AWSaqua} use SSDs attached to FPGAs to implement a caching layer for RedShift that supports SQL filtering operations and operator push-down to minimize the amount of data movement from storage to the processing nodes. All these designs are based on introducing a \textit{bump-in-the-wire} processor to be able to process data closer to here it initially resides, instead of moving it first and then processing it. 

In Farview we adopt a similar design and also use FPGAs as the processing components as it is done in most existing designs \cite{Ibex,Accorda-19,Your-SQl,AWSaqua}, but we require neither changes to the interface towards the storage layer 
% KK: suggest shortening to "changes to the storage layer interface"
nor specialized processors. Unlike Amazon's AQUA, we disaggregate memory and treat it not as intermediate caching layer but simply as an extension of the memory used to keep the buffer pool. 
% KK: above, you argue for a design that disaggregates the buffer pool from the query processing nodes; here you argue that disaggregated memory is an extension of the buffer pool memory, which seems inconsistent. (It's also not clear where the main buffer pool is, that's being extended.)
The choice of FPGAs is aligned with the growing trend to use them for hardware acceleration in the cloud (e.g., Microsoft Catapult \cite{catapult1.0,catapult2.0,catapult3.0}).


\subsection{RDMA}

RDMA allows using the network protocol (InfiniBand~\cite{infiniband}, RoCE~\cite{roce})
and the Network Interface Card (NIC) to move data directly between different machine memories. This is accomplished by using DMA features
that allow the NIC to read and write from and to the host memory directly \cite{RDMA-patterns}. At the speed at which networks operate today, they are no longer considered as much a
a bottleneck as before and they can efficiently transfer large amounts of data across machines at the rates
of DRAM memory channels~\cite{galakatos2016end}. %That makes the network an attractive component to use for  systems as it can significantly increase performance, but on the other hand it also requires systems to be redesigned in a way that they can take advantage of the network capabilities. However, if systems are carefully designed, 
RDMA can be used to great effect in databases \cite{DPI}, and it has been shown to speed up distributed operators such as data shuffling \cite{Blanas-RDMA}, joins~\cite{barthels2015rack, barthels2017distributed},
transactional workloads~\cite{Barthels-VLDB20}, or indexing~\cite{ziegler2019designing}. In Farview, we use RDMA to efficiently
transfer data through the network and also to implement a smart NIC that supports SQL operators that act on the RDMA data streams directly on the data path connecting the disaggregated memory to the network, thereby reducing the latency even further by avoiding data transfers to a processor.  

\subsection{Variations on Far Memory}

% KK: although it's important to include these related references around remote/disaggregated/far memory, this discussion seems disconnected from the problem setup above. Since we've already talked about disaggregation and the issues of independent resource scaling above, it's not necessary to re-define and re-iterate those issues here.

The notion that memory and storage can be active, rather than passive, components and can be shared across a cluster of machines
have been around for decades~\cite{TreadMarks96,ActivePages98,IDisks98,IRAM97,PatRAM97}.  
% KK: this statement blurs the line between active/passive~\cite{ActivePages98,IDisks98,IRAM97,PatRAM97} and DSM-style solutions~\cite{TreadMarks96}; suggest separating the reference lists, and adding things like~\cite{Farm14,Grappa15,Hotpot17} to the DSM list. 
However, as mentioned data grows and applications become
memory hungry making DRAM a major bottleneck in data centers~\cite{FacebookNVM18, GoogleFarMemory19}.
To address this need, approaches leverage advances in memory technologies and networking to increase effective DRAM capacity.
Within a local node, studies have explored compressing cold pages into local DRAM~\cite{GoogleFarMemory19} or
using local NVM directly as memory or with DRAM acting as a transparent caching layer~\cite{Octane19,Octane19-b,HybridMem16}.
In a distributed setting, memory (DRAM or NVM) made available through the network is generically referred to as
\textit{Far Memory}~\cite{FarMemory19}. If the memory is attached to a regular computing node,
it is referred to as \textit{Remote Memory}. If the memory is an independent device detached from a computing node,
it is called \textit{Disaggregated Memory}.  
% KK: the combination of these sentences plus the next three paragraphs seems like a lot; perhaps pare back to a single sentence with the three terms here, and let the subsequent paragraphs define the terms and discuss their pros/cons.

\textit{Remote memory} is a shared, distributed memory infrastructure where a group of comparably equipped
(e.g., with a processor, local memory, local storage) compute nodes make their memory available to their peers.
This organization has the advantage of not requiring any additional resources and, theoretically, improves resource
utilization by taking advantage of unused memory across a group of machines. However, remote memory has several potential drawbacks such as 
the entanglement of compute and memory capacity and the expansion of the failure domain and attack surface of each machine,
leading to application failures and vulnerabilities~\cite{GoogleFarMemory19, RemoteMemory17}. 

% : a) it does not allow scaling compute and memory capacity independently, thereby increasing cost; b) it does not increase the memory capacity if all servers are active at the same time~\cite{Blades09}; c) it assumes the memory in other machines is unused, which is not always true, and makes managing the overall availability including tail latency, a difficult problem~\cite{GoogleFarMemory19}; d) it expands the failure domain and attack surface of each machine, leading to application failures and vulnerabilities~\cite{GoogleFarMemory19, RemoteMemory17}. 

% the rising popularity of in-memory workloads such as machine learning, key-value stores, and in-memory analytics has caused memory demands in compute clusters to grow rapidly~\cite{Barroso18}. Such a demand, coupled with the slowdown of device scaling~\cite{Lee16}, has led to

% This organization has the advantage of not requiring any additional resources and, theoretically, improves resource utilization by taking advantage of unused memory across a group of machines. 
%\cite{TreadMarks96,RemoteMemory17,FarMemory20}, i.e., 
% Previous systems have presented remote memory to applications as a remote paging device~\cite{FarMemory20, Infiniswap17}, as a file system~\cite{RemoteMemory18}, and as distributed shared memory~\cite{Farm14, Grappa15, Hotpot17}.

\textit{Disaggregated memory} systems use network attached memory that is distinct from the memory in the compute nodes~\cite{Dis12}. 
Disaggregated memory can be scaled independently of the computing or storage capacity of the system~\cite{Blades09}. As a result, it offers the possibility of increasing the efficiency of clusters and data centers by removing the need for memory over-provisioning at each computing node (or by adding unnecessary computing nodes only for their memory). It is easier to allocate, share and manage than memory residing in machines that are also performing other computations. Furthermore, data can be easily encrypted (as we will show) to address the security concerns around remote memory.

% ~\cite{GoogleFarMemory19} when the data is stored in machines where other users are running active computations.

% Previous disaggregated architectures have presented their memory as byte-addressable regions that preserve the load/store interface of conventional memory (e.g., The Machine from HPE~\cite{TheMachine1,TheMachine2}, which uses Gen-Z~\cite{GenZ,Knebel19} rather than RDMA), as a paging device~\cite{Blades09,Dis12}, as a persistent key-value store (e.g., FlatStore~\cite{FlatStore20}, Clover~\cite{pDPM20}), as a database storage engine~\cite{Binnig16}, as a persistent memory file system (e.g., Octopus~\cite{Octopus17}, Orion~\cite{Orion19}), or as recoverable persistent data structures (e.g., AsymNVM~\cite{AsymNVM20}).

% KK: might want to frame these as smarter network-attached memory
As another emerging direction, \textit{far memory}~\cite{FarMemory19} proposes hardware extensions
(e.g., indirect addressing modes, scatter/gather support) to reduce the number of network traversals
to access non-local memory, as well as support for efficient notifications to facilitate consistency of data in local memory.
% KK (from ASPLOS submission): should we also include LITE from SOSP17?
HyperLoop~\cite{Hyperloop18}, AsymNVM~\cite{AsymNVM20}, and StRoM~\cite{Strom20} extend one-sided operations on RDMA smart NICs to include additional system-level and application-level logic.
HyperLoop offloads group-based operations to RDMA NICs to support traditional storage functions like replicating data and managing replicated logs. AsymNVM offloads point-to-point persistent memory allocation, concurrency and transaction functionality.
StRoM offloads point-to-point memory access operations like indirect addressing for remote data structure traversal, data shuffling, and cardinality estimation to support distributed key-value store applications.

All this related work points to the many design choices available when building disaggregated memory. In Farview we combine many of these ideas into a novel design that is tailored to database engines. An important contribution of Farview is to demonstrate that the idea of disaggregated memory is especially suitable to database engines, as it can be combined with the way query plans are run and the semantics made to match the notion of database views. This makes the integration of disaggregated memory a more natural step than in other applications, where the interface or access to memory needs to be changed or even the way memory is managed changes completely (e.g., by presenting it as a key-value store). 
% KK: suggest dropping "or even the way that memory is managed changes completely"

==> chapters/earlier_versions/farview-v1.tex <==
\section{Farview}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/system.pdf}
\caption{Farview system}
\label{fig:system}
\end{figure}

% KK: this section should start with a one-sentence description of what Farview is, not just its interface. Also, seems like "similar to" might prompt the question "if it's similar to, not the same, how is it different?" See below for potential rewrite.
%Farview has been designed with an interface similar to that of a buffer pool in a conventional database architecture. 
%Threads processing queries access base tables by reading them from the buffer pool and copying the data to its private working space. 
%In Farview, the buffer pool is implemented as disaggregated memory supporting operator offloading and accessible through RDMA. 
%For the query thread, nothing changes except that a read operation is not over local memory, but over RDMA to the disaggregated memory. In what follows we describe the implementation of Farview: the underlying interface, the FPGA design, the smart NIC component, as well as the supported operators. 

Farview is a smart disaggregated memory with operator offloading capabilities that behaves as a buffer pool in a conventional database architecture.
Traditionally, query processing threads access base tables by reading them from the buffer pool and copying the data to their private working space.
With Farview, nothing changes for the query thread, except that the read operation is not to local memory, but over RDMA to the disaggregated memory, potentially with a subset of the operators already applied. 
In what follows we describe the implementation of Farview: the interface it presents, the FPGA design, the smart NIC component, and the supported operators. 

%is a % platform for prototyping 
%smart disaggregated memory that exposes a \textbf{DK: What should be the new notion here?} view API over the stored data providing a way to dynamically offload the memory operators. The view API provides
%a flexible set of operators, categorized into smart scanning, selection, aggregation and system support operators. All these can be remotely executed with minimum overhead. Farview is implemented on top of \textit{Coyote}~\cite{korolija2020coyote}, an FPGA shell with smart NIC capabilities and virtualized memory support. Farview extends one-sided RDMA verbs to raise the level of abstraction provided by the disaggregated memory. In the following sections, we describe the views API and provide an overview of the Farview architecture and its operators.

\subsection{Data API}

Farview exposes the data stored on smart disaggregated memory through a coherent set of pipelined operators that support various queries and
% KK: what do you mean by "coherent" -- just that it's the standard query processing pipeline that's used by most analytic queries? if so, this might be a logical place to put the operator pipeline figure.
different operator data types. Different combination of operators are pre-compiled into high-performance hardware circuits. These form specialized operator pipelines that can be dynamically off-loaded to the disaggregated memory and into the Farview during runtime. The operators and their pipelines can easily be modified, extended and new ones can easily be added by combining the existing ones or changing their parameters. They thus present a good compromise between high performance and flexibility.

Farview currently implements a range of hardware operators needed for commonly executed queries. The operators can be categorized in the following manner: (1) \textit{smart scanning} operators supporting sophisticated forms of addressing and memory access; These operators are able to expose the data stored on smart disaggregated memory through a set of non-materialized views that present data to users in logical representations rather than in the way the data is physically stored. (2) \textit{selection} operators producing only the data matching a given collection of predicates and filtering out the unneeded elements; (3) \textit{aggregation} operators that combine the information across the query; (4) \textit{system support operators} that perform data processing in-situ before or in lieu of sending the data. We demonstrate seven operators in these categories, including strided memory traversals, projection, predicate-based selection, regular expression matching, distinct, group by and encryption/decryption. 

Farview exposes a simple high level query data API to the clients. Upon the establishment of the connection to the remote back-end node, the clients are provided with the created object representing it (\textit{QPair}). This object holds all the necessary information for a specific connection and is passed to any of the subsequent Farview methods (see Section~\ref{subsection:net_stack}). The available back-end operators providing a variety of operator pipeline combinations can be dynamically loaded and exchanged. This swap is in the order of milliseconds, depending on the size of the allocated query pipeline regions~\cite{korolija2020coyote}.

The following function is used for this purpose:

\begin{lstlisting}
bool loadFarView(QPair *qp, FView *fv);
\end{lstlisting}

The memory in the back-end is virtualized. It can also be shareable between clients and in this case it is allocated from a preallocated shared buffer. Since we are focusing on read-only scenarios there is no concurrency control. Memory for tables can simply be allocated with the following allocation functions:

\begin{lstlisting}
bool allocTableMem(QPair* qp, FTable *ft);
void freeTableMem(QPair *qp, FTable *ft);
\end{lstlisting}

Regular RDMA requests for simple reading/writing to the remote buffer table can be sent with the following two functions:

\begin{lstlisting}
void rdmaRead(QPair* qp, FTable *ft, uint64_t src_offs, uint64_t dst_offs, uint64_t size);
void rdmaWrite(QPair* qp, FTable *ft, uint64_t src_offs, uint64_t dst_offs, uint64_t size);
\end{lstlisting}

The actual base Farview request corresponds to a specialized RDMA verb (based on RDMA Write) that invokes the remote processing operation with an arbitrary parameter set specific to each operator pipeline. This generic function is used as the basis for building additional interfaces supporting higher levels of abstractions such as queries.

\begin{lstlisting}
void farView(QPair* qp, FTable *ft, uint64_t *params);
\end{lstlisting}


\subsection{System overview}

Prototyping smart disaggregated memory requires several components, including DRAM, memory controllers, a network stack, a mechanism to support concurrent access to the memory, and a smart NIC capable of running operators acting either on the memory accesses or the data being transferred. Modern FPGAs, which offer flexibility in design, are equipped with a growing amount of local FPGA-attached memory \cite{u250} (e.g., up to 512 GB on some experimental systems~\cite{Enzian20}). This memory provides far better performance than memory which has to be accessed over PCIe. Multiple banks are usually present offering additional parallelization potential, a crucial advantage in the type of workloads targeted by Farview whenever data is filtered and thus not sent over the network. We leverage this design flexibility and implement Farview on an FPGA, as shown in Figure \ref{fig:system}. Section~\ref{sec:eval} provides more details of our experimental setup.
%Farview leverages this flexibility to implements these components on an FPGA, 
%Modern FPGAs are usually equipped with a growing amount of local, FPGA attached memory \cite{u250} and some experimental systems have announced up to 512 GB of local memory on the FPGA \cite{Enzian20}. 
%(\todo this is one of the aspects that would be different in a real, disaggregated implementation). As it is common in such designs (e.g., Intel's HARP or Amazon F1 instances), Farview contains a fixed region where we deploy the Farview infrastructure (network stack, memory controllers, etc.) and a reconfigurable region where we deploy the operators.

To manage concurrent connection flows, Farview uses multiple \textit{virtual dynamic regions} on the FPGA, each implementing a separate set of operators, conforming to each of the connections. These regions are dynamically reconfigurable, the logic deployed in them can be changed at run time without having to reconfigure the whole FPGA. These dynamic regions are part of the operator stack. They are placed between the network stack and the memory stack and are provided with standard interfaces to both.

The network stack manages all external connections and RDMA requests. It identifies flows using \textit{queue-pairs}, information that is used internally as well as to route the flow of requests and data through Farview accordingly. For networking we use an open source RoCE v2, 100 Gbs network stack \cite{Strom20} that we have adapted and extended. Section~\ref{subsection:net_stack} describes this stack in more detail.

The memory stack houses the memory management unit (MMU) which handles all address translations to dynamically allocated memory on the FPGA containing the tables, allowing each client to use optimally one or more of the available memory channels. It provides the necessary arbitration as well as isolation between concurrent accesses by different client processes.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/view.pdf}
\caption{View in a dynamic region}
\label{fig:view}
\end{figure}

Figure \ref{fig:view} illustrates the operation of a single dynamic region. As described in the previous section, the Farview API provides both the standard one-sided RDMA read/write commands to read or write data from/to memory and a Farview verb, implemented as a one-sided operation that invokes the loaded operator over the read or write data stream. A request is processed as follows. First, the request's virtual address and transfer length parameters are forwarded to the memory controller (the blue path in Figure \ref{fig:region}). If the request is a simple RDMA read/write request, it contains no additional parameters. If the request is a Farview verb, it carries a number of operator-specific parameters (green path). Control of the memory access patterns for operators takes place in the Farview addressing operator which permits different striding access patterns. The write path allows RDMA updates to the memory. The view data processing occurs along the read RDMA data path. Responses to these requests containing necessary network meta information are sent through the response channel (green path). With this architecture, views can dynamically control and influence the size of the response data transfers. This enables the implementation of filtering, for instance, where the size of the filtered data is unknown prior to the processing. The direct data streams between memory controller, view and the network are sized in such a way to saturate the available bandwidth of each module and to provide optimal performance.

\subsubsection{Network Stack}
\label{subsection:net_stack}

The network stack we use implements a reliable RDMA connection protocol. We extend the original stack with support for out-of-order execution at the granularity of single network packets since this is an important feature in a disaggregated memory setting. The original stack implements regular one-sided InfiniBand verbs: RDMA write and RDMA read. Similar to other remote memory systems based on RDMA, (e.g., \cite{AsymNVM20}), we add an additional Farview one-sided verb to control the operators. It includes a number of additional parameters containing the necessary signals to the disaggregated memory on how to access and process the data. The network stack manages connections, buffers, and keeps the necessary state while remaining highly customizable so that it can support further extension to how disaggregated memory operates. It exposes a defined set of streams corresponding to each connection flow and each dynamic region.

In RDMA, the information describing a single node to node connection or RDMA flow is associated with a \textit{queue pair}. The queue-pairs contain unique identifiers which are used to differentiate the flows and to provide the isolation through a series of hardware arbiters. Upon connection establishment, each flow and its corresponding queue pair gets associated to one of the dynamic regions. The operator (or operators) corresponding to the specialized requested view can be loaded into the dynamic region, and the flow is then ready to be processed. Queue pairs are also used to keep track of the dynamically allocated  memory locations used in the RDMA requests between remote nodes. This allocated memory can be shared between different queue-pairs.

\subsubsection{Memory Stack}
\label{subsection:mem_stack}

The central part of the memory stack is the memory management unit (MMU) responsible for all memory address translations to a shared dynamically allocated memory. It propagates and routes all memory requests and subsequent data. It supports the issuing of multiple outstanding requests and has fully decoupled read and write channels. It provides parallel interfaces, isolation and protection for all the requests stemming from different dynamic regions with a set of arbitrators, crossbars and dedicated credit-based queues.
 
The MMU contains a translation lookaside buffer (TLB) implemented with the fast on-chip memory. In Farview, it is software loaded from the host CPU and it holds all virtual to physical address mappings for the dynamic regions. The memory allocation is dynamic and is handled by the Linux kernel driver module with a pool allocator. This allocation is invoked remotely by the client with the API functions. The control of the MMU can be done either by a small external CPU or by the same FPGA with one of the \textit{softcore} CPUs directly implemented in the FPGA fabric \cite{microblaze}.

Farview's MMU supports naturally aligned 2 MB pages. This greatly reduces the coverage problem of smaller pages.
%(an observation shared with the design of Optimus \cite{HyperFPGA20}). 
Farview's MMU also abstracts the memory channels and banks. It provides a transparent abstraction for DRAM accesses that maximizes the available DRAM bandwidth by aggregating the bandwidth from multiple channels (if present). It does this by allocating the memory in striping pattern across all available memory channels~\cite{korolija2020coyote} thus maximizing the available bandwidth to each application region. The higher bandwidth wich is available to each dynamic region also permits the vectorization model of the processing~\ref{sec:vectorization}.

\subsubsection{Operator Stack}
\label{subsection:oprator_stack}

The operators deployed in the dynamic regions are written against the interfaces exposed by the Farview's network and memory stacks. They are portable across Farview deployments, regardless of the underlying FPGA. The operators have clearly defined set of interfaces based on simple handshaking logic~\cite{axi} which makes it easy to combine the existing ones in arbitrary fashion. They are written in common hardware description languages like VHDL or Verilog,  as well as in high level synthesis tools such as Vivado HLS which offers a C++ like syntax to the users. 

Operators can use a number of available hardware resources, such as dedicated on-chip memory with very low random access latency (BRAM, URAM) or specialized DSP blocks for floating-point computation. The only restriction is to conform to the provided set of interfaces. The operator pipelines function as bump-in-the-wire processors where they can process the incoming and outgoing data directly without adding too much overhead thus producing significant performance increase.

The operator stack is where this smart logic attached to each connection flow to/from memory is deployed. It is implemented as a collection of pre-defined dynamic regions where logic can be deployed at run time and swapped on-the-fly without affecting the integrity and operation of the system or other operators. These regions and their access to memory are isolated from each other (see Section~\ref{subsection:mem_stack}). 
Such functionality is typically not available in commercial systems, but very often studied in the literature, e.g.,  \cite{AmorphOS,HyperFPGA20,VirtualFPGA20}. Compared to existing FPGA frameworks, in Farview the regions have to be connected to the network and memory stacks, reducing the degrees of freedom in placement and sizing. Linking dynamic regions to an actual network stack is different from linking them to the Ethernet (PHY and MAC) connector(s) available in the FPGA. 
%\todo\textit{We might even go for the removal of this part completely.} 
%For instance AmorphOS \cite{AmorphOS} does not consider the network at all, neither as a physical connector nor as a network stack. Optimus \cite{HyperFPGA20} and ViTAL \cite{VirtualFPGA20} do virtualize the Ethernet connector but only at the physical level, %The latter just connects the regions to the Ethernet interface without any arbitration of the access to that interface 
%as this is enough to communicate across FPGAs using point-to-point links in a ring topology without going through a network switch \cite{VirtualFPGA20}. 

Due to the spatial architecture of FPGAs, elements with a fixed location like the memory controller, and especially large ones like the network stack, pose significant challenges in the design. 
%In Farview the dynamic regions need to be connected to logical elements (RDMA queue pairs) rather than to a given hardware module and these connections need to be mapped rather than \textit{wired} as they can change at run time. %Additional differences between existing systems and Farview is that 
Farview always places logic between the RDMA stack and the memory controller as the only purpose of the system is to implement a smart NIC rather than arbitrary functionality. The management infrastructures in Farview have to cope with network line rates of 100 Gbps and even higher internal ones, something that requires at least 512 bit wide buses \cite{Strom20,Limago19} and introduces quite a few restrictions on the placement of the regions and the ability to give them arbitrary sizes. Hence the choice of pre-defined regions. 

\subsection{Operator pipeline}

The operator pipeline sends the data requests to the memory and handles the actual query data processing. Each pipeline and the surrounding logic is part of the dynamic regions belonging to a single client process at a time. The reconfigurable nature of these regions adds a large level of flexibility as it allows virtually unlimited number of different operator combinations and types to be supported by the system. Each of the operator pipelines processes one tuple every cycle. In this paper all data is stored in row-order format, however there is nothing intrinsic preventing the support for column-order data which only requires column-order operators.

Once the query request arrives, it is first forwarded to the smart scanning addressing operator outputs the correct access pattern in the main memory. At the same time and necessary parameters for the actual processing are forwarded to the operator data pipeline. Once data starts arriving from the memory it enters the data pipeline where it is processed in a streaming fashion. Once the processing is done, the data is sent over the network. This way, the overhead of the processing can be efficiently hidden behind the memory and network operations. The figure~\ref{fig:} shows an example of an operator pipeline with some of the possible locations for each of the operators. In the following sections we explain the operators in more details.

\subsubsection{Smart scanning}

Many applications access data neither entirely sequentially nor completely at random. For instance, databases traverse large tables looking at particular attributes located in memory at regular intervals form each other. Such applications would benefit from a strided access interface. Scientific applications use strided access when performing column-major accesses to data stored in row-major order.
%The same when traversing large data collections where we are interested only in a few items placed at regular intervals. 
To support queries like these, each dynamic region in a Farview has an addressing operator which can read arbitrary spaced memory locations as if they were continuous thus providing a large number of different data views to the clients. This operator is the one responsible for the issuing of the main memory requests. Different kinds of smart addressing operators are supported, ones doing striding access patterns, scatter gather techniques or indexing addressing operators accessing the data in completely random patterns. In the paper we present the striding operator, which has the main purpose of creating non-materialized views without inferring the extra memory overhead.
The specific striding interface exposes the following parameters: 1) \textit{Size}, the size of a single element, 2) \textit{Count}, the number of elements to fetch, 3) \textit{Stride}, the offset between elements. Any combination of these values is supported. 

\subsubsection{Parsing}

The first part in the data operator pipeline is the parsing module. This module reads the incoming data stream, parses it depending on the supplied information describing the tuples and their size and finally outputs tuples into the pipelines for further processing. During the parsing the tuples are annotated with information obtained from the parameter queues submitted in the original query request. These parameters are simple flags which state, e.g., which of the columns are part of the selection or projection. They interpretation entirely depends on the actual combination of operators being used.

\subsubsection{Selection}

The first operator after the parsing stage is the selection which directly maps to the \texttt{WHERE} SQL clause, for example in queries of the form: \texttt{SELECT * FROM T WHERE T.a > 50}. This operator has the ability to greatly reduce the amount of data for the processing of later stages and ultimately the overall amount of data sent through the network thus reducing the overall network bandwidth usage. We choose to hard-wire the selection predicate matching circuit instead of creating a truth table as done in~\cite{ibex} as Farview has the ability to dynamically exchange the operators. This approach uses less resources and, at the same time, support a variety of different possible predicates. Besides this, it also permits combined complex predicates between different tuple columns which can even be split into multiple pipelined cycles. The annotations from the parser determine which of the columns in the tuple are evaluated during the predicate matching phase.

\subsubsection{Vectorization}
\label{sec:vectorization}

The processing of a single tuple at a time, as found in the volcano model~\cite{}, can lead to the underutilization of the available network bandwidth, especially in the cases where the selectivity of the data is low leading to only some of the data being forwarded over the network. To utilize the bandwidth of the network more efficiently, in these cases the vectorized processing model can provide optimization on the memory side which possesses a far larger amount of memory bandwidth. The optimization exposes a larger read interface to each of the dynamic regions permitting faster reading speeds. This is possible in Farview through the combination of already mentioned memory striping and parallelization of the operator pipelines. In this case, the parser emits more than one tuple into parallel data pipelines which allows higher read bandwidths from the main memory. When selectivity is low, the throughput at the output of the pipelines is lower, thus at the same time utilizing more of both the network and memory bandwidths. The Figure \ref{fig:vectorization} shows the example of a selection data pipeline with 2 parallel pipeline vectorization.

\subsubsection{Regular expression matching}

Farview provides increasing advantages as the computational complexity of the filtering increases. To demonstrate this, we integrate an open source regular expression library for FPGAs \cite{regex17} into Farview and use it to read strings from the disaggregated memory. This can be advantageous for queries that have complex \texttt{LIKE} predicates (e.g. TPC-H Q16). In these operators data is retrieved from the remote node only when it matches the given regular expression. The operator implements regular expression query acceleration with multiple parallel engines, instantiated in the FPGA in such a way which allows it to fully sustain the processing line rate. Unlike software solutions, the performance of the operator is dominated by the length of the string and does not depend on the complexity of the target regular expression.

\subsubsection{Distinct}

The distinct operator eliminates repeated column entries before they can be sent over the network. It directly maps to the \texttt{DISTINCT} SQL clause, in queries such as: \texttt{SELECT DISTINCT T.a, T.b FROM T}. It does this by hashing the values and preserving the entries in the hash tables present in the fast FPGA on-chip memory. As the complete hashing is calculated in the FPGA the distinct operation can be done on multiple columns without noticeable performance overhead and with a price of increased FPGA resources.

To be able to sustain the line rate and not negatively affect the overall pipeline processing, the operator needs to be fully pipelined and to overcome the latency of the lookups and updates of the implemented hash table. This creates data hazards as the successive tuples with the same keys will not see mutual updates. To approach this problem we apply some of the strategies explained in~\cite{Ibex} with the main difference being the far higher line rate that we have to sustain in our work (over 40 times greater) which yields additional design constraints.

To guarantee full pipelining and constant lookup times the hash table that we implement does not handle collisions. In the case of collisions they are written in a buffer and the system fallbacks to the software solution for these specific cases. To greatly reduce the amount of possible collisions we implement a form of cuckoo hashing~\cite{} with several hash tables which can all be looked up in parallel. Upon the eviction from one of the tables, the evicted entry is inserted into the next hash table with a different function. This occurs fully in the background and does not affect the full pipelining of the operator.

To successfully hide the latency of the hash table a cache holding most recent keys is implemented. The cache needs to be a true LRU(\textit{Least Recently Used}) cache in order to guarantee the protection from possible data hazards. The standard implementations of LRU caches come with a lot of overhead as pointers and extra history keeping data structures need to be present. For this reason, we implement the cache with a shift register which adds a certain amount of the latency to the data streams (the amount depends on the number of the cuckoo hash tables), but is able to efficiently provide a quick lookup. The nature of the shift register provides a true LRU replacement policy and this solution thus fully satisfies the strict requirements imposed by Farview. The architecture of the distinct operator presenting our design choices is shown in the Figure~\ref{fig:}.

\subsubsection{Group by}

In many applications, data is often read and grouped to perform some form of aggregation (e.g., sum or average). Operations like these directly map to the \texttt{GROUP BY} SQL query clause. It can support queries such as: \texttt{SELECT COUNT(T.a), T.b FROM T GROUP BY T.b}. The operator doing these operations is supplied in the Farview. The structure is quite similar to the distinct operator and most of the design choices and difficulties they overcome remains here as well. The implemented cache in this case is write-through as it is no longer sufficient to just discard the data prior to sending it. The operator reads the complete table and all of it's tuples without sending anything over the network until the full aggregation is handled. At the same time it inserts the distinct entries into a separate queue. Once the aggregation is done, the queue is used to lookup and flush the entries from the hash table along with the aggregation results to the network. The architecture of the group by operator is shown in the Figure~\ref{fig:}.

\subsubsection{Projection and sending}

At the end of the processing pipeline, the annotated columns are first projected based on their annotation flags. To reduce the overall data sent over the network multiple columns across the tuples are packed into 64 byte words prior to their writing into the output queue. An overflow buffer is used to achieve this whilst sustaining the line rate. In case of the vectorized processing model, the tuples are first consumed from each of the parallel pipelines with the simple round-robin arbiter. 

The sender unit is the final step before the results are emited to the network stack. It monitors the output queue and issues the packet commands necessary for the packet header information in the network stack. The dynamic way of handling the RDMA commands by the sender unit allows us to create RDMA commands even when the final data size is not known a priori, as is the case with most of the operators.

\subsubsection{Encryption/decryption}

A key concern for both remote memory and smart disaggregated memory is the need for data encryption \cite{GoogleFarMemory19}. Farview implements encryption so that the data is treated similarly to Microsoft's Cypherbase \cite{Cypherbase15}, where a database stores only encrypted data but can still answer queries over such data by using an FPGA as a trusted module. We have implemented encryption as an operator using 128-bit AES in counter mode. Since the AES module is fully parallelized and pipelined, it can operate at full network bandwidth. This means that no throughput penalty is paid when this operator is applied on the stream, incurring only a negligible overhead in latency. This allows the data to be stored securely. Because no real processing penalty is induced, encryption can be placed at multiple spots in the overall system architecture. Similarly one could provide additional system support operators such as compression, decompression, etc.

==> chapters/earlier_versions/introduction-2021-02-18.tex <==
\section{Introduction}

Historically, databases have invested significant efforts to reduce the I/O overhead, with I/O being broadly construed. Initially, such an overhead was clearly defined: memory was very limited in capacity and disks were slow. Over time, the bottleneck changed in nature as faster storage became available (SSDs, NVM), memories became larger, and multicore emerged as the dominant processor design. Yet, the I/O overhead remains a major factor in the overall performance. To minimize this overhead, databases have relied on keeping more and more data in memory, a trend that cannot continue due to two main reasons: databases induce a lot of data movement, which is known to be a major source of inefficiency in modern computing; and the amount of data to be processed keeps growing while DRAM capacity is not. % and (3) the distributed nature of cloud and data center computing makes the coupling of storage, compute, and memory capacity very problematic from a cost and efficiency point of view. 

Optimized query plans typically push down selection and projection operators to filter out the base tables as early as possible. 
However, the step of going from base tables to the data actually needed by the query is an expensive one. Base tables are fetched from storage as blocks that are placed in a buffer cache in memory. From there, a query thread reads the data and filters it
to form the input to the rest of the query plan. Often, most of the data is 
dropped because it does not match the query's selection predicate. As more data is involved, the overhead becomes larger. Data movement has been identified as one of the biggest sources of inefficiencies in computer designs \cite{dally2011power,dally2020domain}, making the way databases operate intrinsically problematic from a systems perspective even if main memory could be grown indefinitely.

As the size of analytical databases keeps growing, databases are confronted with a widening gap between the size of the working set and the DRAM available. This is also true in the cloud in general, where DRAM capacity has become a major limitation due to the growth of in-memory data analytic applications \cite{GoogleFarMemory19}. NVM has been introduced as an alternative that is both cheaper and has higher capacity than DRAM (and persists data) but has larger latency. In databases, it has been proposed as way to increase virtual memory capacity using NVM as fast local storage~\cite{neumann2020umbra}, to offload parts of the engine~\cite{van2019persistent}, build DBMSs on top of NVM \cite{arulraj2019non, arulraj2017build}, or use combinations of DRAM, SSD and NVM to offload different components to each storage layer \cite{van2018managing, arulraj2019multi}. Such designs typically modify and expand the memory hierarchy through NVM but inherently make the problem of data movement worse. Working at the level of virtual memory does not address the overhead of potentially moving
large amounts of data to the CPU, just to have most of it filtered or projected out. The issue is so nowadays pressing that even
new hardware between the memory and the CPU has been proposed to filter data 
as early as possible to minimize bus congestion and cache pollution \cite{OracleM716,Accorda-19}.

In this paper we argue that a possible solution to these issues is to exploit the growing distributed nature of database engines, particularly in the cloud and data centers, where the system architecture favors scale-out designs. In such distributed settings, the coupling of storage, compute, and memory capacity is very problematic from a cost and efficiency point of view. Not being able to independently provision each one of those elements leads to inefficiencies due to over-provisioning. For instance, allocating large amounts of memory for tasks that are not compute heavy leaves CPU unused as other applications might not be able to run on the remaining memory. Conversely, allocating many virtual CPUs to a task may result in the memory being underutilized for lack of compute capacity for other tasks. This is why essentially all cloud architectures follow a clear trend towards disaggregation. Currently, the most visible form of disaggregation is the separation of compute and storage. The next step is the disaggregation of memory and compute, which is being pursued in different forms: far or remote memory~\cite{RemoteMemory17,Farmemory19,FarMemory20}, far persistent
memory~\cite{AsymNVM20}, disaggregated memory~\cite{Blades09,gao16,Dis12}, smart remote memory~\cite{Strom20}, etc. This memory can be in the form of either disaggregated Non-Volatile Memory (NVM) \cite{AsymNVM20} or DRAM~\cite{Blades09,Dis12} or in using the DRAM on
other machines~\cite{RemoteMemory17,RemoteMemory18} with even the first operating systems to manage such disaggregated systems starting to appear \cite{Legos18}.

In this paper we demonstrate that databases are uniquely positioned to exploit disaggregated memory and that it can be used to address both the issues in provisioning DRAM capacity and of inefficient data movements. Our approach is based on physically detaching query processing from memory buffer management. The buffer pool can be placed on disaggregated memory accessible through the network, with query processing nodes provisioned on demand to run a query by reading the data from the network attached buffer pool. The advantages of such a design are obvious. 
Consider, for example, queries with large selectivity (e.g., TPC-H Q6) 
or an aggregation after a \texttt{GROUP BY} statement. In the first case, the database has to fetch a large amount of data into the buffer cache
just for the query to discard most of it, leading to unnecessary data movement. In the second case, a query of the form
\texttt{SELECT T.a, COUNT(*) FROM T GROUP BY T.a} will usually
return only a handful of tuples, but it still requires transferring and scanning the entire table. The smart disaggregated memory we propose offers the opportunity to (1) avoid keeping a large buffer cache in all computing nodes by centralizing it in disaggregated memory and (2) push down operators to the disaggregated memory so that the processing nodes receive only the relevant data. Since the processing nodes do not maintain the buffer cache, the memory allocated to them can be smaller. To a certain extent, what we propose is conceptually similar to Amazon's AQUA \cite{AWSaqua}, which also mirrors earlier designs on smart storage \cite{Ibex,Your-SQL}, where FPGAs are used to push down SQL filtering and aggregation to network attached SSDs to reduce unnecessary data movements. While AQUA works as an intermediate cache between storage and the analytics engine (Redshift), we propose to do something similar at the buffer pool level. Such a redesign has to be done carefully, otherwise the flexibility so gained  will come at a high cost of increased data movement and network data transfer overheads. 

%The problem is not unique to data processing and, as a result, there is a
%growing interest in ways to expand memory systems:  In the context
%of databases, the DRAM bottleneck has driven database designers to expand in-memory databases with fast local storage~\cite{neumann2020umbra, lerner2020takes} (a model similar to that of ~\cite{GoogleFarMemory19} but tailored to databases), Non-Volatile Memory~\cite{haas2020exploiting, arulraj2017build},
%or combinations of different memory systems~\cite{vogel2020mosaic}. For network attached storage, the added latency is compensated by using
%RDMA~\cite{galakatos2016end} and/or smart NICs~\cite{KVdirect,Strom20}, as RDMA
%offers lower latency and lower overheads than TCP/IP \cite{Binnig16}. In fact, the
%interplay between network and smart remote memory is seen as a crucial factor in
%the performance of future cloud computing
%architectures~\cite{lerner2020networking}.


%only receive and process the relevant data. 

%, an operation that can be easily offloaded to the disaggregated memory
%such that we don't have to transfer the whole table \texttt{T} from the main memory in case of a row store or the
%column \texttt{T.a} in case of a column store. Although we present only two simple examples, a large number of
%queries apply some form of aggregation and/or selection so that they can show only the relevant
%results to the user, making more eminent the need to offload such simple computations rather to a smart memory component than to the CPU.

% Some of these ideas are focused on new forms of memory such as Non-Volatile Memory (NVM) \cite{AsymNVM20} while others are focused on DRAM \cite{}. Similarly, some assume network attached memory in the form of either NVM or DRAM \cite{Blades09,Dis12} while others focus on using the DRAM on other machines \cite{RemoteMemory17,RemoteMemory18}. In most cases, the added latency incurred by having to go through the network is compensated by using RDMA \cite{} and/or smart NICS \cite{KVdirect,Strom20}, as RDMA offers lower latencies and lower overheads than TCP/IP.

To prove that these ideas can be made to work in practice, we have developed \textit{Farview} (FV), a novel platform for data processing over disaggregated memory. %We focus on disaggregated memory in the form of DRAM because it offers an interesting alternative design point to using NVM, which is more associated to storage. Farview is intended as a large pool of main memory available through the network to processing nodes who then do not need to be provisioned with large local memory capacity. 
% KK: "interesting alternative design point to using NVM..." <- this point isn't substantiated (NVM is already being used as memory, so I'm not sure reviewers will buy the claim that it's more associated with storage)
% KK: "large pool of main memory": "main memory" could be confusing to readers, who might expect that to be in the local node. Say "large pool of shared memory" instead?
Farview supports near-data processing to compensate for the added latency of accessing memory through the network and also to further reduce the memory needed at the computing nodes by moving data reduction operators (selection, projection, aggregation, etc.) to the disaggregated memory.  The existing prototype of Farview is based on a smart NIC built on top of an open source FPGA shell~\cite{korolija2020coyote} that enables the FPGA to support dynamic operator push down on concurrent streams reading from memory. %These regions can all independently and concurrently access the local virtualized memory and communicate through RDMA. 
The smart NIC supports RoCE v2 at 100 Gbps in the form of an open source RDMA stack \cite{Strom20}, optimizing the interaction between network and memory as well as minimizing the network processing overheads on the computing node CPU, thereby freeing processing capacity. The
interface currently offered to the database is that of a data buffer pool in a conventional database architecture. That is, Farview acts as a disaggregated memory buffer pool that interacts with storage using blocks/pages, 
% KK: this is the first mention of storage, which seems jarring; might be better to lead with the byte-addressable interface presented to the rest of the engine 
but it is byte addressable towards the rest of the engine (the threads running queries at smaller processing nodes). %The design enables an architecture where the data buffer cache is stored in disaggregated memory and made available through RDMA to computing nodes where the queries actually run. 
As an initial use case, we explore data analytics and discuss in detail both the architectural options as well as query execution strategies that can benefit from Farview. For reasons of space, we focus on the design, architecture, and experimental evaluation of Farview when running queries, leaving other aspects such as cache replacement policies to later work.

Farview currently supports a wide range of query operators, from selection and projection to group by and regular expression matching, and including compression and encryption. All these operators achieve near line-rate speed, adding insignificant latency to baseline network overheads. 
%on top of the network one. 
The platform also supports concurrent access, with multiple clients all accessing the same shared disaggregated memory. The experiments show that Farview induces almost no overhead over operating on local memory and provides significant performance gains when data can be reduced in the disaggregated memory, which is the case in most analytical queries 

%In addition to these results, the main contributions of the paper are:

%\begin{itemize}
%    \item A discussion of how the upcoming notion of disaggregated memory can be used in a database engine.
%    \item Showing that near-data processing can be combined with disaggregated memory to compensate for some of overheads of operating over the network.
%    \item The design of Farview combining an FPGA, Smart-NIC, RDMA, as well as the ability to support concurrent access operations over the memory.
%    \item An extensive performance evaluation measuring the impact of disaggregated memory and showing that, maybe counter-intuitively, Farview can often be faster than accessing local memory.
%\end{itemize}

%Database engines have a decades long story exploring distributed architectures and different combinations of storage, memory, and compute to optimize the underlying computing infrastructure to the task at hand. Today, classic designs based on shared memory, shared nothing, or shared disks approaches have found their counterparts in the cloud and data centers where data processing remains one of the main applications. For instance, it is fair to say that, in the cloud, the separation of storage and compute is a given, providing a design that mirrors the shared disk architectures found in many database engines. Even cloud native databases (Aurora \cite{} or Snowflake \cite{}) naturally exploit the separation by designing the system to take advantage of it. Such a separation provides much more flexibility to both the storage and compute layers in terms of architecture, optimization, and where to place the data. It allows the storage to take care of aspects such as scalability and availability in a way that is orthogonal to the compute layer. It also allows the compute layer to be provisioned independently of the storage layer, an extreme form of this idea being data processing on serverless platforms \cite{Lambada,Starling,Hellerstein}. The added latency caused by the network in between storage and compute is often compensated with near-data processing (most cloud storage layers today allow some form of data processing at the storage layer to reduce the amount of data moved) and/or through explicit caching layers (e.g., Amazon AQUA \cite{}). A trend also explored in research (e.g., \cite{Ibex,YourSQL,Caribou,...}) and that is likely to continue unabated.




==> chapters/farview.tex <==
\section{Farview: System Overview}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/system.pdf}
\caption{High level view of Farview's architecture}
\label{fig:system}
\end{figure}

% KK: this section should start with a one-sentence description of what Farview is, not just its interface. Also, seems like "similar to" might prompt the question "if it's similar to, not the same, how is it different?" See below for potential rewrite.
%Farview has been designed with an interface similar to that of a buffer pool in a conventional database architecture. 
%Threads processing queries access base tables by reading them from the buffer pool and copying the data to its private working space. 
%In Farview, the buffer pool is implemented as disaggregated memory supporting operator offloading and accessible through RDMA. 
%For the query thread, nothing changes except that a read operation is not over local memory, but over RDMA to the disaggregated memory. In what follows we describe the implementation of Farview: the underlying interface, the FPGA design, the smart NIC component, as well as the supported operators. 

Farview is a smart disaggregated memory with operator offloading capabilities that behaves as a database buffer
pool. Traditionally, query processing threads access base tables by
reading them from the buffer pool and copying the data to their private working space. With Farview, nothing
changes for the query thread, except that the read operation is not on local but remote on the disaggregated memory,
potentially with a subset of the operators already applied. 

%is a % platform for prototyping 
%smart disaggregated memory that exposes a \textbf{DK: What should be the new notion here?} view API over the stored data providing a way to dynamically offload the memory operators. The view API provides
%a flexible set of operators, categorized into smart scanning, selection, aggregation and system support operators. All these can be remotely executed with minimum overhead. Farview is implemented on top of \textit{Coyote}~\cite{korolija2020coyote}, an FPGA shell with smart NIC capabilities and virtualized memory support. Farview extends one-sided RDMA verbs to raise the level of abstraction provided by the disaggregated memory. In the following sections, we describe the views API and provide an overview of the Farview architecture and its operators.

% Farview exposes the data stored on smart disaggregated memory through a coherent set of pipelined operators that support various queries and different operator data types. 
% KK: what do you mean by "coherent" -- just that it's the standard query processing pipeline that's used by most analytic queries? if so, this might be a logical place to put the operator pipeline figure.

\subsection{Basic architecture}

Prototyping smart disaggregated memory requires several components, including DRAM, memory controllers,
a network stack, a mechanism to support concurrent access to the memory, and processing capacity for
operator push-down. Modern FPGAs are a natural match for such functionality as high performance and flexibility can all be combined
in a single device rather than having to connect separate components such as processor, NIC, and memory. 
FPGAs can also support substantial amounts of local memory (even High Bandwidth Memory)~\cite{Enzian20}.
Farview's design %(Figure~\ref{fig:system}) 
leverages these characteristics to implement disaggregated memory as a lean component.
%Farview has been ported to several FPGA boards (see Section \ref{sec:eval} for details).

Inside the FPGA, Farview is organized around three main modules: the memory stack, the network stack,
and the operator stack (Figure~\ref{fig:system}). The memory stack houses the memory management unit (MMU),
which handles all address translations to dynamically allocated on-board memory attached to the FPGA. It provides the necessary
arbitration as well as isolation between concurrent accesses. The network stack manages all external
connections and RDMA requests, providing fair share mechanisms across all concurrent accesses.
The operator stack contains the dynamic logic necessary to push down operators to the disaggregated memory.
It lies between the memory and the network stack and it can be seen as a specialized stream processor
acting on the data as it moves from the memory stack to the network stack. It also controls
how the data is retrieved from the memory stack. The operator stack is reconfigurable and the logic inside can be changed at runtime.

In Farview, the buffer pool is implemented in the memory stack. It can be used as regular memory
with blocks/pages being loaded from storage as needed. Farview allows optimizing the memory layout
to maximize the memory bandwidth (e.g., by spreading the data across memory channels). The process of
mapping the incoming data pages to the chosen layout is automated as one more operator and it is
transparent to the rest of the system. In what follows, we will refer to the threads processing actual
queries at computing nodes as clients. Clients access the disaggregated memory through the network
stack. Access requests indicate the operator or operators to apply to the data as it is read. These
operators are deployed in the operator stack as either isolated operators or operator pipelines. Like
it is done in conventional query processing, operator pipelines are constructed from predefined
building blocks that implement a given operator and provide standard interfaces to combine operators
into pipelines. We also assume that the clients have local catalog information that is used to determine
the addresses of the tables to be accessed. 

%, due to their high performance, flexibility of programming, and substantial local FPGA-attached memory~\cite{u250} (e.g., up to 512 GB on some experimental systems~\cite{Enzian20}).


%Farview is implemented using an FPGA platform. 

\subsection{SQL operators}

Operators can be written using common hardware description languages like VHDL or
Verilog but also in the C++-like syntax supported by high-level synthesis tools
such as Vivado HLS. Individual operators have well-defined interfaces and can be combined
with other operators to form an \op, which is compiled and then deployed to a dynamic region
at runtime. Operators are specific to Farview, and are not tied to a particular FPGA board. This makes the operators portable across different Farview deployments and across different boards. This is achieved by using standardized interfaces
across all elements of the design. 

%Farview enables operator push down, supporting the operators that are needed for analytic queries, as shown in Figure~\ref{fig:pipeline} \todo{insert pipeline figure here}.
The operators currently implemented include: (1) \textit{smart scanning} operators supporting
sophisticated forms of addressing and memory access, which expose the data stored on smart
disaggregated memory in a logical representation (e.e., a view) rather than in the way the data is
physically stored and can be used for projection; (2) \textit{selection} operators that filter data according to a collection
of predicates; (3) \textit{grouping} operators that combine tuples; and (4)
\textit{system support operators} that process data in-situ before sending the data (currently encryption/decryption). 
% DK: The smart scanning is the place where we can mention that this operator can be used for projection.

%We demonstrate seven operators in these categories, including strided memory traversals, projection, predicate-based selection, regular expression matching, distinct, group by and encryption/decryption. 

\subsection{Deploying operators}
%FPGAs are spatial architectures where sharing implies using parts of the available real state. 
To deploy operators that can process data on the disaggregated memory, the FPGA is divided
into multiple \textit{virtual dynamic regions} that operate concurrently.
Each dynamic region deals with an access request to the disaggregated memory and implements a separate
\op. These regions are dynamically reconfigurable: the logic deployed in them can be swapped at runtime
without having to reconfigure the whole FPGA. This swap takes in the order of milliseconds, depending
on the size of the allocated query pipeline regions~\cite{korolija2020coyote}.
These dynamic regions  are placed between the network stack and the memory stack, utilizing standard interfaces to both.

Different combinations of operators can be precompiled into hardware designs forming operator
pipelines (e.g., a selection and then an aggregation). These pipelines are dynamically
loaded into the FPGA during run time at the client's requests. The operators and their pipelines
can easily be modified or extended, and new ones can easily be added by combining the existing ones or
changing their parameters. This approach is a compromise between high performance and flexibility
but, as pointed out, mirrors the way query plans are built in conventional engines.
% DK: I think this one explains it well, we should try to get across that the pipelines do not support just one query, there is some flexibility in them (for instance which columns are used for selection and do on).


% KK: add short discussion of concurrent operation here?

%In what follows we describe the implementation of Farview: the interface it presents, the FPGA design, the smart NIC component, and the supported operators. 
%In the remainder of this section, we describe the Farview platform in more detail and present the operators it implements.
% KK: stretch goal:, and provide an illustrative example of how Farview processes a query.

\section{Farview: Implementation}

Farview is implemented on top of an open source FPGA shell~\cite{korolija2020coyote}. The shell provides a layer of abstraction hiding services like RDMA network stack, memory virtualization, and concurrent system users behind high level interfaces. 

\subsection{Architecture}

Whenever a remote query request to the Farview node is made, it is first routed from the network stack to the correct virtual dynamic region in the operator stack belonging to the client that initiated the request. To obtain one of the available dynamic regions the clients open up a connection with the Farview node. The request is processed in the dynamic region and the actual read request is forwarded to the memory stack. This request contains the virtual address and the size of the data to be fetched. The memory stack maps this to the physical addresses and issues requests to the on-board FPGA memory. The returned data is streamed back to the dynamic region where processing by specific loaded operators can be applied. Finally, the data is forwarded to the network stack and the results are sent directly to the memory of the client. 

The interfaces of the data and the requests are all based on a simple \textit{AXI stream} handshaking protocol~\cite{axistream} which provides uncomplicated synchronization, pipelining, and backpressure mechanisms, all allowing the Farview nodes to support processing at high throughput. The standard interfaces help with  portability across different boards as the dynamic region where the operators are loaded always exposes the same set of the interfaces to the operators, thereby simplifying the task of creating the operators. This protocol also allows deep pipelining of the overall design which allows processing to occur simultaneously in different areas of the system. 

All of the stacks and all of the internal stack stages in Farview have their specific spatial positions inside FPGA fabric. The stacks thus need to be physically connected to transfer the data. To attain high frequencies and reduce the impact of the physical distance between the stacks, the data is buffered in queues as it traverses from one stack to the other. The queues are implemented using fast on-chip FPGA memory. This memory is used in Farview for buffering and for any of the temporary states created by Farview operators. The buffering allows clear decoupling of processing stages. It helps with structuring the overall system and allows Farview nodes to achieve the operating frequencies necessary to sustain processing at line rate speeds. The frequencies of the components in the Farview range between 250 (network stack, operator stack) and 300 MHz (memory stack). 


\subsection{Memory stack}
\label{subsection:mem_stack}

%\todo{@Dario: Add some numbers of the bandwdith and latency of the memory on the FPGA. Indicate it is similar to that available on the CPU except that there are no caches. Explain the 18GBps that appears in the figure. Indicate that in the boards we are currently using, there are 4 channels but boards like the 280 can have as many as 32 channels. Explain, with a pointer to Coyote, that Farview can separate memory regions and ensure access controls.}

The central part of the memory stack is the memory management unit (MMU), which is responsible
for all memory address translations to a shared dynamically allocated memory. It propagates and
routes all memory requests and subsequent data. It supports the issuing of multiple outstanding
requests and has fully decoupled read and write channels. It provides parallel interfaces,
isolation and protection for all the requests stemming from different dynamic regions with a
set of arbitrators, crossbars, and dedicated credit-based queues.
 
The memory stack accesses the DRAM memory organized in multiple channels which are attached to the FPGA chip. The "softcore" memory controllers for these channels are instantiated in the FPGA fabric and take physical space inside the FPGA. Each memory channel can provide a certain amount of memory bandwidth. In our case, we use the Alveo u250~\cite{u250} which has up to four separate memory channels. For the tests in this paper we utilized up to two of these. Each of these requires its own softcore controller that runs at 300 MHz. The width of the interface to the memory channel controller is 64 bytes. This implies a maximum theoretical bandwidth of ~18 GBps per channel (Figure~\ref{fig:system}). The bandwidth matches those usually found on more conventional systems with general purpose CPUs~\cite{Binnig16}. Boards like the Alveo u280 can also contain separate high bandwidth memory (8 GB) which is able to deliver a much larger total bandwidth ($\sim$300 GBps). We leave the integration of Farview with this memory for future work.
 
The MMU contains a translation lookaside buffer (TLB) implemented on BRAM
(the fast on-chip FPGA memory as opposed to DRAM which is outside the FPGA chip
in a regular memory module). Farview's TLB holds all virtual-to-physical
address mappings for the dynamic regions. 

%The memory
% KK: is this statement correct?
%allocation is dynamic and is handled by the Linux kernel driver module with a pool allocator. This allocation is invoked remotely by the client with the API functions. The control of the MMU can be done either by a small external CPU or by the same FPGA with one of the \textit{softcore} CPUs directly implemented in the FPGA fabric \cite{microblaze}.
% KK: so the TLB is software-loaded from the host CPU, but the control of the MMU can be managed by a softcore CPU in the FPGA?
% GA: I have commented this out. For what we are proposing, there is no CPU and the configuration of memory is different than from what we were doing in ASPLOS.
Farview's MMU supports naturally aligned 2 MB pages. This greatly reduces the coverage problem of smaller pages.
%(an observation shared with the design of Optimus \cite{HyperFPGA20}). 
The memory stack uses the DRAM attached to the FPGA. Multiple channels are usually present, offering additional parallelization potential. Farview's MMU also abstracts the memory channels. It provides a transparent abstraction for DRAM accesses that maximizes the available DRAM bandwidth by aggregating the bandwidth from multiple channels (if present). It does this by allocating the memory in a striping pattern across all available memory channels~\cite{korolija2020coyote}, thus maximizing the available bandwidth to each application region. The higher bandwidth available to each dynamic region also enables a vectorized processing model (described in Section~\ref{sec:vectorization}).

\subsection{Network stack}
\label{subsection:net_stack}

%\todo{@Dario: Explain the 12GBps that appears in the figure. Mention the packet based arbitration and what it does. You might also want to briefly explain how the data is written back to the client's memory (just mention that this is a step in the RDMA protocol that identifies where in the memory of the client the data will be written).}

Farview's network stack implements a reliable RDMA connection protocol, building on an existing
open source stack~\cite{Strom20} that implements regular one-sided RDMA read and write verbs. 
We extend the original stack with support for out-of-order execution at the granularity of single
network packets.
The out-of-order execution along with credit based system and packet based processing allows the Farview to provide the fair-sharing, an important feature in a system shared by multiple separate clients concurrently. Crucially it prevents any malevolent behaviour by any of the users which could lead to a complete system stall. 

% KK: it's not immediately obvious why out-of-order execution is important only for disaggregated memory settings
%The original stack implements regular one-sided InfiniBand verbs: RDMA write and RDMA read. 

In RDMA, the information describing a single node-to-node connection or RDMA flow is associated with
a \textit{queue pair}. Farview identifies flows using such \textit{queue pairs}, information that is
used internally as well as to route the flow of requests and data through the system. The queue pairs
contain unique identifiers which are used to differentiate the flows and to provide isolation through
a series of hardware arbiters. Upon connection establishment, each flow and its corresponding queue pair
gets associated with one of the dynamic regions. The \op corresponding to the flow
is loaded into the dynamic region, and the flow is then ready to be processed. Queue pairs are also used to keep
track of the dynamically allocated  memory locations used in the RDMA requests between remote nodes. This dynamically allocated memory can also be shared between different queue pairs. It is virtual and client sends the virtual address of the local client buffer where data results will be loaded by one-sided RDMA operations from Farview. The client node needs to be equipped with a commercial NIC which supports same RDMA protocol. 

Similar to other remote memory systems based on RDMA, (e.g., \cite{AsymNVM20}), we add an additional
Farview one-sided verb, based on RDMA write, to control the operators. It includes a number of additional parameters containing
the necessary signals to the disaggregated memory on how to access and process the data. The network
stack manages connections, buffers, and keeps the necessary state, while remaining highly customizable
so that it can support further extensions. Each network connection is assocaiated with one virtual dynamic region and in turn with one data stream from disaggregated Farview memory stack. This stream passes through the same dynamic region where direct processing on it can occur.

% KK: TODO: it would be useful to clarify what streams exist per connection flow, how a connection relates to a dynamic region (next para. handles the connection:region mapping). All of this should be made clear, relative to the lines in Fig. 2.

Compared to existing FPGA frameworks (which support arbitrary functionality), in Farview's smart NIC
the dynamic regions must be connected to the network and memory stacks, which have fixed locations
within the FPGA, thus reducing the degrees of freedom in placement and sizing. Farview's management
infrastructure must cope with network speeds of 100 Gbps (and even higher internal speeds), which
requires wide buses (at least 512 bit)~\cite{Strom20, Limago19}, further restricting region placement and sizing.
We choose pre-defined dynamic regions to accommodate these placement and sizing restrictions. In practice this
implies that the size of each virtual dynamic region is fixed and cannot be changed. However, each region
is more than large enough for the purposes of offloading the operators we intend to support. The 100 Gbps also presents the maximum bandwidth that the network stack can sustain ($\sim$12 GBps in Figure~\ref{fig:system}). This bandwidth is significantly slower than the maximum available bandwidth of the memory stack. For this reason a number of operators that filter data and reduce network bandwidth usage can lead to higher overall performance as they can bridge the gap between these bandwidths (reading faster and more than sending).

\subsection{Operator stack}
\label{subsection:oprator_stack}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/view.pdf}
\caption{Single dynamic region in the operator stack}
\label{fig:op_stack}
\end{figure}

The operator stack is where the \ops attached to 
connection flows to/from memory are deployed. 
%An operator pipeline effectively functions as a bump-in-the-wire that processes the incoming and outgoing data directly without adding too much overhead.
%, thus producing significant performance increase.
The stack is implemented as a collection of predefined dynamic regions. 
The operators deployed in the dynamic regions use the interfaces exposed
by Farview's network and memory stacks. %They are portable across Farview deployments, regardless of the underlying FPGA. 
% KK: does "They" refer to the network and memory stack APIs, or the operators themselves (or both)?


%The operators have a clearly defined set of interfaces based on simple handshaking logic~\cite{axi}, which makes it easy to combine the existing ones prior to complation in an arbitrary fashion. 
% KK Q: this makes it sound like the APIs support operator chaining, but so far we've only looked at operator fusing.

\OP logic can be deployed and swapped on-the-fly without affecting the integrity and
operation of the system or other operator pipelines belonging to other clients. These regions and their access
to memory are isolated from each other (see Section~\ref{subsection:mem_stack}). 
Such functionality is typically not available in commercial systems, but very often studied in
the literature, e.g.,~\cite{AmorphOS,HyperFPGA20,VirtualFPGA20}. 

Figure \ref{fig:op_stack} illustrates how a single dynamic region processes a request. The base RDMA read and write requests
forward the virtual address and transfer length parameters directly to the memory
stack and to the MMU (the blue path in Figure \ref{fig:op_stack}), bypassing the dynamic region. If the request is a simple RDMA
read/write request, it contains no additional parameters. If the request is a Farview command,
it carries a number of operator-specific parameters (green path), along with information about the virtual memory locations it is accessing. The number of parameters can vary depending on the specific operators that are present in the \OP. For example, control of
the operator memory access patterns takes place in the Farview addressing operator, which
permits different striding access patterns and projections. The write path allows RDMA updates to the memory. The
operator bump-on-the-wire data processing occurs along the read data path. The width of the input of this path to the dynamic region scales with the number of available memory channels. This way, each dynamic region gets full bandwidth potential of the disaggregated memory and its multiple memory channels. This is possible via aforementioned striping technique. The output is forwarded to the network stack and its width is 64 bytes, same as the provided network interface. This is enough to fully saturate it.

Responses to these requests containing the resulting data are sent via the response channel (green path).
% Responses to these requests containing necessary network meta information are sent through the response channel (green path). 
With this architecture, operators can dynamically control and influence the size of the response data transfers. This enables the implementation of filtering, for instance, where the size of the filtered data is unknown prior to processing. The direct data streams between the memory controller, the operator, and the network are sized in such a way to saturate the available bandwidth of each module and to provide optimal performance.

%\todo{@Dario: explain the bandwidth available at each layer. Figure  already refers to them anyway}
% KK: note: I replaced "view" with "operator" above.
% KK: not exactly clear what the last sentence (sizing direct data streams to provide optimal performance) means


\subsection{Client interfaces}

%\todo{@Dario: This needs concrete examples of how a query is executed and invoked. The current description is too abstract}

Farview exposes a simple high level data API, which provides both the standard low level one-sided RDMA read/write commands to read or write data from/to memory and an extra Farview command, implemented as a one-sided operation that invokes the loaded operator(s) over the read data stream. This command is used as a base on top of which more complex SQL commands can be implemented.

Clients begin by establishing a connection to the Farview node.
In response, the client is provided with a created object representing the connection (\textit{QPair}), which holds all the necessary information for the connection and is used as an argument to subsequent Farview methods. The following function is used for this purpose:

\begin{lstlisting}
bool openConnection(QPair *qp, FView *node);
\end{lstlisting}

Farview memory is virtualized, and can be shared between Farview clients.
Since we are focusing on read-only scenarios, Farview does not currently provide concurrency control. Clients allocate memory for tables using the following allocation functions:
% KK: how important is the preallocated shared buffer? Is this different than how memory would be allocated for a single client's access?

%The memory in the back-end is virtualized. It can also be shareable 
%% KK: not sure "back-end" is a good term
%between clients and in this case it is allocated from a preallocated shared buffer. Since we are focusing on read-only scenarios there is no concurrency control. Memory for tables can simply be allocated with the following allocation functions:

\begin{lstlisting}
bool allocTableMem(QPair* qp, FTable *ft);
void freeTableMem(QPair *qp, FTable *ft);
\end{lstlisting}

Regular RDMA requests for simple reading/writing of the remote table can be sent with the following two functions:

\begin{lstlisting}
void tableRead(QPair* qp, FTable *ft);
void tableWrite(QPair* qp, FTable *ft);
\end{lstlisting}

Farview's request corresponds to a specialized RDMA verb that invokes the remote processing capabilities with an arbitrary parameter set specific to each operator pipeline. The following generic function is used as the basis for building additional higher level functions supporting specific operator combinations and queries:
%higher levels of abstractions such as queries.

\begin{lstlisting}
void farView(QPair* qp, FTable *ft, uint64_t *params);
\end{lstlisting}

As an example of a possible higher level function we present a selection operator with real number predicates: 

\begin{lstlisting}
void select(QPair* qp, FTable *ft, uint64_t *projection_flags, uint64_t *selection_flags, float predicate);
\end{lstlisting}

This function can be used for the following type of queries:

\begin{lstlisting}[language=SQL]
SELECT S.a FROM S WHERE S.c > 3.14;
\end{lstlisting}

In this case, the projection flags variable would signal column \texttt{a} whilst the selection flag would signal column \texttt{c}. The predicate would be passed as a value. More complex variations are possible. For instance, if the hardware operator supports it, the predicate operation could also be a variable.

The interface presented here is not supposed to be used by the client, but by the query compiler intended for Farview. The query compiler is part of the future work in the project.

%\todo{code should be generated by the query compiler, future work.}

\section{Farview: Operators and pipelines}

\subsection{Operator Pipeline} 
\label{sec:OP}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/pipeline1.pdf}
\caption{{\OP}}
\label{fig:pipe1}
\end{figure}

An \op contains one or more operators that handle the actual query data processing.
It effectively functions as a bump-in-the-wire that processes the incoming data
from disaggregated memory directly. As the processing is done in pipelines in a streaming fashion there is not much overhead present. 
Each \pipe is deployed into a dynamic region that belongs to a single client process at a time.
% KK: todo: should define operator pipeline earlier 
The reconfigurable nature of these regions adds a large level of flexibility, as it allows an arbitrary
number of different operator combinations and types to be natively supported by the system. Which operators are actually present in the pipeline depends on the requested query. In one scenario the pipeline can support projection, followed by selection and group by. In another it can support operations on strings such as regular expression matching where we can for instance also assume that the data is stored in encrypted format, thus requiring prior decryption in the pipeline.

Each pipeline has the potential to be fed with input data every single FPGA clock cycle. In the same manner, it has the potential to produce results on the output of every cycle. This design allows a lot of the processing to be fully hidden behind memory operations. In the query terms this translates to the pipelines being fed with a single tuple in each cycle at max.\footnote{We assume that all data is stored in row format, but there is nothing intrinsic preventing the support for column data.} % which only requires column-order operators.
% KK Q: each operator pipeline processes one tuple each *FPGA* clock cycle? If you want multiple tuples per cycle per region, you use multiple pipelines in parallel?
% KK: todo: figure out what the most important points are about operator pipelines, and revise the above.

Farview implements a range of operator classes that can be combined into \ops such as the example shown in Figure~\ref{fig:pipe1}, including smart scanning (used for projection), selection, aggregation, and system support operators. 
Once a query request arrives, it is first forwarded to the smart scanning operator, which makes the appropriate access request to the memory stack. %outputs the correct access pattern in the main memory. 
At the same time, any necessary parameters for additional processing are forwarded to the operator data pipeline. 
% KK: todo: need to define operator data pipeline somewhere
Once data starts arriving from the memory, it enters the data pipeline, where it is processed in a streaming fashion. 
Once the processing is done, the resulting data is sent over the network. This way, the overhead of the processing can be efficiently hidden behind the memory and network operations. 
%The figure~\ref{fig:} shows an example of an operator pipeline with some of the possible locations for each of the operators. 


%Prototyping smart disaggregated memory requires 
%several components, including DRAM, memory controllers, a network stack, a mechanism to support concurrent access to the memory, and a smart NIC capable of running operators acting either on the memory accesses or the data being transferred. 
%Modern FPGAs are a natural match for this functionality, due to their high performance, flexibility of programming, and substantial local FPGA-attached memory~\cite{u250} (e.g., up to 512 GB on some experimental systems~\cite{Enzian20}).
%Farview's design, shown in Figure~\ref{fig:system}, leverages these FPGA characteristics.
%(Section~\ref{sec:eval} provides additional details of our implementation platform.)
%This memory provides far better performance than memory which has to be accessed over PCIe. Multiple banks are usually present offering additional parallelization potential, a crucial advantage in the type of workloads targeted by Farview whenever data is filtered and thus not sent over the network. 
% KK: moved this memory info to the memory stack discussion below
%We leverage this design flexibility and implement Farview on an FPGA, as shown in Figure \ref{fig:system}. 
%Farview's FPGA-based design, shown in Figure~\ref{fig:system}, leverages this design flexibility and local memory. 

%Farview leverages this flexibility to implements these components on an FPGA, 
%Modern FPGAs are usually equipped with a growing amount of local, FPGA attached memory \cite{u250} and some experimental systems have announced up to 512 GB of local memory on the FPGA \cite{Enzian20}. 
%(\todo this is one of the aspects that would be different in a real, disaggregated implementation). As it is common in such designs (e.g., Intel's HARP or Amazon F1 instances), Farview contains a fixed region where we deploy the Farview infrastructure (network stack, memory controllers, etc.) and a reconfigurable region where we deploy the operators.


%Section~\ref{subsection:oprator_stack} describes the operators the dynamic regions implement in more detail.




%, a crucial advantage in the type of workloads targeted by Farview whenever data is filtered and thus not sent over the network. 

% KK: what's not clear is whether FPGA memory is the disaggregated memory OR whether it's merely the working memory for the individual operators within each region. Fig. 1 makes it seem like the former; Fig. 2 makes it seem like the latter.

% KK: since we're no longer looking at reduced precision, do we need to talk about DSP blocks for FP computation?

%Operators can use a number of available hardware resources, such as dedicated on-chip memory with very low random access latency (BRAM, URAM) or specialized DSP blocks for floating-point computation. The only restriction is to conform to the provided set of interfaces. 

% KK: I really hacked away at the material after this point, to hone in on what seemed (to me) to be the main issue. Please feel free to fix, if I broke it.
% KK note: this paragraph used to be connected to the dynamic reconfigurability discussion and mention of commercial systems/research literature


%Linking dynamic regions to an actual network stack is different from linking them to the Ethernet (PHY and MAC) connector(s) available in the FPGA. 
%%\todo\textit{We might even go for the removal of this part completely.} 
%%For instance AmorphOS \cite{AmorphOS} does not consider the network at all, neither as a physical connector nor as a network stack. Optimus \cite{HyperFPGA20} and ViTAL \cite{VirtualFPGA20} do virtualize the Ethernet connector but only at the physical level, %The latter just connects the regions to the Ethernet interface without any arbitration of the access to that interface 
%%as this is enough to communicate across FPGAs using point-to-point links in a ring topology without going through a network switch \cite{VirtualFPGA20}. 

%Due to the spatial architecture of FPGAs, elements with a fixed location like the memory controller, and especially large ones like the network stack, pose significant challenges in the design. 
%%In Farview the dynamic regions need to be connected to logical elements (RDMA queue pairs) rather than to a given hardware module and these connections need to be mapped rather than \textit{wired} as they can change at run time. %Additional differences between existing systems and Farview is that 
%Farview always places logic between the RDMA stack and the memory controller as the only purpose of the system is to implement a smart NIC rather than arbitrary functionality. The management infrastructures in Farview have to cope with network line rates of 100 Gbps and even higher internal ones, something that requires at least 512 bit wide buses \cite{Strom20,Limago19} and introduces quite a few restrictions on the placement of the regions and the ability to give them arbitrary sizes. Hence the choice of pre-defined regions. 

% KK: todo: get a consistent list of the operators that are supported, so that we can say it up front. Also point out that a DB-savvy FPGA programmer can add more?
% Farview currently implements strided memory traversals, projection, predicate-based selection, regular expression matching, distinct, group by and encryption/decryption.

\subsection{Vectorization}
\label{sec:vectorization}

Early database systems were processing data using the Volcano or tuple-at-a-time model~\cite{graefe1990encapsulation}.
Although this model has advantages such as ease of implementation and cache locality for certain categories of queries (e.g. 
\texttt{SELECT S.a, S.b FROM S WHERE S.a > 20}), it has a large overhead because of the \texttt{next()} function calls, which
pass tuples from one operator to the next. To alleviate this inefficiency, the database community came up with query compilation
~\cite{neumann2011efficiently} and column stores or combinations of both. Column stores either process data in full batches like
MonetDB~\cite{boncz2008breaking}, or in
smaller vectors like VectorWise~\cite{zukowski2012vectorwise}. The latter allows the use
of tight loops and/or SIMD instructions to process column data, allowing DBMSs to take advantage of the latest CPU advances
for data processing. In Farview, we use a model similar to the vectorized model of Vectorwise, but with the main difference that
the size of the vector is smaller and not necessarily as large as possible to fit the L1 cache. Our vectorized model is possible 
through the combination of memory striping (described above) and parallelization of the operator pipelines. 
With vectorization, the parser module can parse the tuples faster and emit them into paralllel data pipelines. This allows both higher read bandwidths from the main memory and higher processing throughput to be achieved. The vectorization example for the \OP performing vectorized projection and selection is shown in Figure~\ref{fig:pipe2}.

% KK Q: when you say parallel data pipelines, do you mean multiple independent one-tuple-at-a-time pipelines, each processing one of the tuples?
%When selectivity is low, the throughput at the output of the pipeline is lower, thus at the same time utilizing more of both the network and memory bandwidths. 
% KK: not sure this makes sense to me -- vectorization makes good use of the memory bandwidth, by requesting multiple tuples at a time; if you have multiple pipelines running in parallel, you can consume multiple tuples each cycle. How does this improve network bandwidth usage?

% KK: suggest deferring vectorization performance to the results section, along with all other results
% Figure \ref{fig:vectorization} shows the example of a selection data pipeline with 2 parallel pipeline vectorization.

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/pipeline2.pdf}
\caption{{Vectorization}}
\label{fig:pipe2}
\end{figure}


\subsection{Smart Scanning Operators}
Many applications access data neither entirely sequentially nor completely at random. For instance, databases
traverse large tables looking at particular attributes located in memory at regular intervals from each other.
Consider for example a projection in a row store of the form \texttt{SELECT S.car, S.price FROM S} where
\texttt{S.car, S.price} are non-consecutive attributes that have a number of attributes of fixed length between them. 
In certain scenarios where tables hold a large number of tuples in between the performance would greatly benefit from a strided access interface where only the necessary attributes are fetched effectively doing a projection.  
% Scientific applications use strided access when performing column-major accesses to data stored in row-major order.
%The same when traversing large data collections where we are interested only in a few items placed at regular intervals. 
To support queries like these, each dynamic region in a Farview has a smart addressing operator, which
can read arbitrarily spaced memory locations as if they were continuous, thus providing a large number
of non-materialized data views without incurring additional memory overheads. By doing this it projects only the necessary attributes.
% KK Q: so, the smart scanning/addressing operator is present in all pipelines?
The smart addressing operator is responsible for issuing data requests to the memory. Different kinds of smart addressing are supported, including striding access patterns, scatter/gather, or indexed addressing that issues requests according to a permutation expressed in an input index array.
%accessing the data in completely random patterns. 
% KK: note: most HPC folks say "strided" rather than "striding"; is "striding" common in the DB community?
%In this paper, we present the striding operator,
%, which has the main purpose of creating non-materialized views without inferring the extra memory overhead.
%whose interface exposes the following parameters: 1) \textit{Size}, the size of a single element, 2) \textit{Count}, the number of elements to fetch, 3) \textit{Stride}, the offset between elements. Any combination of these values is supported. 

Another important step in the data operator pipeline is the projection module. This module reads the incoming data stream,
parses it depending on the supplied information describing the tuples and their size, and finally projects the needed
tuples into the pipeline for further processing. It converts memory interface data to higher level of abstraction represented in tuples. During the parsing, the tuples are annotated with information
obtained from the parameter queues submitted in the original query request. These parameters are simple flags
that state which of the columns are part of the selection, projection or grouping phases. Their interpretation depends on the actual combination of operators being used and their specific implementations.

%\todo{This needs to be turned into the projection operator}
% KK: not sure there are enough details here to really understand how this works; it doesn't seem super-important, though, so I'm not sure it makes sense to add more detail.

% DK: This whole section needs to be shifted towards projection

\subsection{Selection Operators}

The first operator category after the parsing and projection stage is data filtering, which directly maps
to the SQL \texttt{WHERE} clause (e.g., in queries of the form \texttt{SELECT * FROM T WHERE T.a > 50}).
This operator has the ability to greatly reduce the amount of data to be processed by later stages and ultimately the overall
amount of data sent through the network, thus reducing the overall network bandwidth usage. For example in the case of TPC-H Q6,
only 2\% of the data are finally selected, and pushing the filtering to the disaggregated memory reduces the I/O
by orders of magnitude. Selection operators include both predicate selection and a more complex regular expression matching operator.

\textbf{Predicate selection}: For selection involving conventional data types, the value of an attribute
is compared against a constant provided in the query. In FPGAs, such a comparison can be implemented
in different ways. We choose to hardwire the selection predicate as an actual matching circuit instead
of creating a truth table as done in~\cite{Ibex}, as Farview has the ability to dynamically exchange the operators. 
% KK Q: not sure why dynamically exchanging operators suggests a hard-wired circuit; perhaps I don't understand what you mean by hard-wired
This approach uses fewer resources and, at the same time, supports a variety of different possible predicates. It also permits complex predicates defined over different tuple columns, which can be split into multiple pipelined cycles. 
% KK Q: it's not clear whether all complex predicates are split into multiple pipelined cycles, or whether this is optional 
The supplied annotations from the request determine which of the columns in the tuple are evaluated during the predicate matching phase.

\begin{figure}[t]
\centering
\includegraphics[width=0.75\columnwidth]{figures/pipeline3.pdf}
\caption{{Regular expression matching operator}}
\label{fig:pipe3}
\end{figure}

\textbf{Regular expression matching}: String matching is becoming an increasingly important operator in SQL (e.g. using either
\textit{LIKE} predicates like in TPC-H Q16 or regular expression matching). This is even more eminent in unstructured data
types, such as in the case of JSON fields in PostgreSQL. In Farview we have integrated an open source
regular expression library for FPGAs~\cite{regex17} and use it to filter strings. In these operators data is
retrieved from the remote node only when it matches 
% Dejan removed below, it was repeated text
%the given where data is retrieved only when it matches 
the
given regular expression. The operator implements regular expression query acceleration with multiple parallel engines,
instantiated in the operator stack.
% in such a way which allows it 
%% KK Q: parallel engine vs. parallel pipeline?
The regular expression matching is done in parallel processing engines in the regular expression module. The parallelisation allows the module to fully sustain processing at line rate. Unlike software solutions, the performance of the operator is dominated by the length of the string and does not
depend on the complexity of the target regular expression.

\subsection{Grouping Operators}

\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth]{figures/pipeline4.pdf}
\caption{{Distinct operator}}
\label{fig:pipe3}
\end{figure}

\textbf{Distinct}: The distinct operator eliminates repeated column entries before they are sent over the network.
It directly maps to the SQL \texttt{DISTINCT} clause, in queries such as: \texttt{SELECT DISTINCT T.a, T.b FROM T}.
It operates by hashing the values and preserving the entries in the hash tables present in the fast FPGA on-chip memory.
As the complete hashing is calculated in the FPGA, the distinct operation can be done on multiple columns without noticeable
performance overhead, but only with using more FPGA resources.

To sustain the line rate without negatively affecting the overall pipeline processing, the distinct operator
needs to be fully pipelined, to overcome the latency of the lookups and updates of the hash table. This
pipelining creates potential data hazards, in the case where two successive tuples with the same value will be inserted into the hash table and ultimately sent over the network as distinct elements. Because of the latency of the hash table, the second (following) tuple cannot see the update produced by the first one. 
% KK Q: doesn't this just result in a race to insert into the hash table? Or are you also concerned about collisions?
To approach this problem we apply the strategy explained in~\cite{Ibex} by implementing an LRU cache to hide the hash table latency. The main difference
is the far higher line rate that we have to sustain in our system (over 40 times greater), yielding
additional design constraints.
% KK Q: to make the paper self-contained, need to list the strategies from~\cite{Ibex} that we use

To guarantee full pipelining and constant lookup times, the hash table that we implement
does not handle collisions. Instead, collisions are written into a buffer, which is sent to the client
to be deduplicated in software.
%In the case of collisions they are written in a buffer and the system falls back to a software solution for these specific cases. 
To greatly reduce the collision likelihood, we implement cuckoo hashing, with several hash tables
that can be looked up in parallel. Upon the eviction from one of the tables, the evicted entry is inserted into
the next hash table with a different function. This occurs in the background and does not affect the full pipelining of the operator.

To successfully hide the latency of the hash table, we implement a cache to hold the most recent keys.
The cache needs to be a true Least Recently Used (LRU) cache in order to guarantee the protection
from possible data hazards. 
% KK Q: I understand why the cache must be completely up-to-date, but why does LRU replacement suffice? There's no guarantee that data values will be processed in sorted order, so I would think that all values in the cache would be important.
The standard implementations of LRU caches come with a lot of overhead, as pointers and extra
history-keeping data structures need to be present. For this reason, we implement the cache with a shift
register which adds a 
%certain amount of
negligible latency to the data streams (the amount depends on the
number of cuckoo hash tables), but is able to efficiently provide a quick lookup. The nature of
the shift register provides a true LRU replacement policy and this solution thus fully satisfies the
strict requirements imposed by Farview. The design of the distinct operator is shown in Figure~\ref{fig:pipe3}.
% KK Q: what will this figure show? do we have space for it?

\textbf{Group by}: In many applications, data is often read and grouped to perform some form of aggregation (e.g., TPC-H Q1).
Operations like these directly map to the SQL \texttt{GROUP BY} clause (e.g., for queries such as
\texttt{SELECT T.b, COUNT(*) FROM T GROUP BY T.b}). Farview provides a group by operator, with a structure quite similar to
the distinct operator; most of the challenges and design choices exist here, as well. The same cuckoo hash tables are used to preserve the groups. The implemented cache in
this case is write-through, as it is no longer sufficient to just discard the data prior to sending it.
The operator reads the complete table and all of its tuples without sending anything over the network, to perform
the full aggregation. At the same time, it inserts the distinct entries into a separate queue. Once the aggregation
has completed, the queue is used to lookup and flush the entries from the hash table along with any of the requested
aggregation results to the network.
% KK Q: what will this figure show? do we have space for it?

\textbf{Aggregation}: In FPGAs aggregation is simple and these operators can easily be supported either standalone where simple computation are performed directly on the passing data streams or on top of the group by operator where each entry in the hash table contains an additional aggregation result. Farview supports a range of standard aggregation operators like count, min, max, sum and average.

\subsection{System Support Operators}

\textbf{Packing}: At the end of the processing pipeline, the annotated columns are first packed based
on their annotation flags in a bid to reduce the overall data sent over the network. Multiple
columns across the tuples are packed into 64 byte words prior to their writing into the output queue.
This packing uses an overflow buffer to efficiently sustain the line rate. In case of the vectorized processing model, the tuples are first combined from each of the parallel pipelines with a simple round-robin arbiter. 

\textbf{Sending}: The sender unit is the final step before the results are emitted to the network stack. It monitors the queue present in this module where the packed results are written. Based on the status of this queue this module issues specific RDMA packet commands
% KK Q: output queue in the network stack or in the operator pipeline?
necessary for the production of correct packet header information in the network stack. The dynamic way of handling the RDMA commands by the sender module allows us to create RDMA commands even when the final data size is not known a priori, as is the case with most of the operators.

% KK Q: just to be clear: is projection is handled earlier in the pipeline, due to the annotations you do as part of parsing? (If projection is only happening at the end of the pipeline, it seems like there's unnecessary data movement going on.) If the projection happens earlier, then this section seems like it's really about how to efficiently send the results.

%An overflow buffer is used to achieve this whilst sustaining the line rate. 

\textbf{Encryption/decryption}: A key concern for both remote memory and smart disaggregated memory is the need for
data encryption \cite{GoogleFarMemory19}. Farview implements encryption so that the data is treated similarly to
Microsoft's Cypherbase \cite{Cypherbase15}, where a database stores only encrypted data, but can still
answer queries over such data by using an FPGA as a trusted module. We have implemented encryption
as an operator using 128-bit AES in counter mode. Since the AES module is fully parallelized and
pipelined, it can operate at full network bandwidth. This means that no throughput penalty is paid when this operator
is applied on the stream, incurring only a negligible overhead in latency. This allows the data to be stored
securely. Because no real processing penalty is incurred, encryption can be placed at multiple spots in the
overall system architecture. Similarly one could provide additional system support operators
such as compression, decompression, etc.

==> figures/intro_fig.tex <==
\begin{figure*}[t!] 
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=0.9\columnwidth]{figures/1a.pdf}
        \caption{1a.}
        \label{fig:skip_list_diag}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=0.9\columnwidth]{figures/1b.pdf}
        \caption{1b.}
        \label{fig:skip_list_diag}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=0.9\columnwidth]{figures/1c.pdf}
        \caption{1c.}
        \label{fig:skip_list_diag}
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=0.9\columnwidth]{figures/1d.pdf}
        \caption{1d.}
        \label{fig:skip_list_diag}
    \end{subfigure}
    
\vspace{0.2cm}
\label{fig:selection_sbs}
\caption{JUST A PLACE HOLDER.}
\end{figure*}

==> graphs_data_vldb/encryption_thr.tex <==
label       RDMA-READ   RDMA-READ+Encryption
64          0.19        0.18
128         0.39        0.4
256         0.78        0.75
512         1.56        1.55
1k          3.1         2.94
2k          6.24        6.07
4k          11.47       11.52
8k          11.8        11.73
